Optimal Transport-Based Displacement Interpolation with Data Augmentation for Reduced Order Modeling of Nonlinear Dynamical Systems

We present a novel reduced-order Model (ROM) that leverages optimal transport (OT) theory and displacement interpolation to enhance the representation of nonlinear dynamics in complex systems. While traditional ROM techniques face challenges in this scenario, especially when data (i.e., observational snapshots) is limited, our method addresses these issues by introducing a data augmentation strategy based on OT principles. The proposed framework generates interpolated solutions tracing geodesic paths in the space of probability distributions, enriching the training dataset for the ROM. A key feature of our approach is its ability to provide a continuous representation of the solution's dynamics by exploiting a virtual-to-real time mapping. This enables the reconstruction of solutions at finer temporal scales than those provided by the original data. To further improve prediction accuracy, we employ Gaussian Process Regression to learn the residual and correct the representation between the interpolated snapshots and the physical solution. We demonstrate the effectiveness of our methodology with atmospheric mesoscale benchmarks characterized by highly nonlinear, advection-dominated dynamics. Our results show improved accuracy and efficiency in predicting complex system behaviors, indicating the potential of this approach for a wide range of applications in computational physics and engineering.

==> sections/abstract.tex <==
\begin{abstract}
We present a novel reduced-order Model (ROM)
that leverages optimal transport (OT) theory
and displacement interpolation to enhance
the representation of nonlinear dynamics in complex systems.
While traditional ROM techniques face challenges in this scenario,
especially when data (i.e., observational snapshots) is limited, our method addresses these issues
by introducing a data augmentation strategy based on OT principles.
The proposed framework generates interpolated solutions tracing geodesic paths
in the space of probability distributions, enriching the training dataset
for the ROM.
A key feature of our approach is its ability to provide a continuous
representation of the solution's dynamics
by exploiting a virtual-to-real time mapping.
% through regression of the relationship between time and the interpolation parameter.
This enables the reconstruction of solutions at finer temporal scales than those provided by the original data.
% , allowing for more detailed temporal analysis.
To further improve prediction accuracy, we employ Gaussian Process Regression to learn the residual and correct the representation between the interpolated snapshots and the physical solution.

We demonstrate the effectiveness of our methodology with atmospheric mesoscale benchmarks characterized by highly nonlinear, advection-dominated dynamics. Our results show improved accuracy and efficiency in predicting complex system behaviors, indicating the potential of this approach for a wide range of applications in computational physics and engineering.

\medskip
\noindent \textbf{Keywords:} Reduced-Order Models, Data-Driven Modeling, Optimal Transport, Displacement Interpolation, Wasserstein Distance, Computational Fluid Dynamics, Parametric PDEs, Synthetic Data Generation, Nonlinear Dynamics, Atmospheric Flow Simulation.
\end{abstract}


==> sections/conclusion.tex <==
%\section{Conclusions and Perspectives}
%\label{sec:conclusions}

%In this work, we have presented a novel approach for reduced-order modeling of atmospheric flows, leveraging optimal transport theory and displacement interpolation. Our method addresses the challenges of capturing nonlinear dynamics and dealing with limited data in atmospheric simulations. By combining POD with regression and OT-based interpolation, we have demonstrated improved accuracy and efficiency in predicting complex atmospheric phenomena, as evidenced by our results on the rising thermal bubble and density current benchmarks.

%The proposed framework offers several advantages over traditional ROM techniques. It enhances the ability to capture nonlinear dynamics through OT-based interpolation, provides efficient data augmentation allowing for better training of deep learning-based ROMs, and it improves temporal resolution through synthetic snapshot generation.

%While our current results are promising, there are several avenues for future research and potential extensions of this work. One potential direction is the development of an adaptive checkpoint selection strategy. The current method uses a fixed set of checkpoints for interpolation, but an adaptive approach could potentially reduce the number of required checkpoints while maintaining or even improving accuracy. This could involve using error estimators or sensitivity analysis to identify critical points in the solution trajectory where additional checkpoints would be most beneficial \cite{Peherstorfer2015}.

%Future work could explore advanced interpolation and extrapolation schemes to enhance our method. Our method currently relies solely on displacement interpolation between checkpoints. A hybrid approach that combines displacement interpolation with standard interpolation methods could offer a better trade-off between computational cost and accuracy, especially in multi-scale problems common in atmospheric sciences. For instance, displacement interpolation could be used for large-scale transport phenomena, while standard interpolation could handle smaller-scale variations \cite{Majda2003}. Additionally, the emerging concept of displacement extrapolation, which extends geodesics in the Wasserstein space beyond known data points, presents intriguing possibilities. This approach could enable predictions of atmospheric states outside the training data range, potentially advancing long-term forecasting and extreme event prediction.

%Another perspective is to perform the interpolation with respect to a carefully chosen reference configuration, rather than between consecutive snapshots. This approach could be particularly beneficial for periodic or quasi-periodic flows, where a single reference state might suffice for the entire simulation. The challenge here would lie in selecting an appropriate reference state and in efficiently computing the transport plans. Recent advancements in multi-marginal optimal transport could be leveraged for this purpose \cite{Pass2015}.

%The integration of our proposed method with real-time data assimilation techniques presents another significant research direction. By continuously updating the ROM with new observational data, we could improve long-term prediction accuracy and adapt to changing atmospheric conditions. This integration could be particularly valuable for operational weather forecasting systems, bridging the gap between model predictions and real-world observations \cite{Blum2009}.

%Finally, while our current work focuses on 2D atmospheric flows, extending the method to 3D scenarios and incorporating additional physics (e.g., moisture, radiation) would be a natural next step. It's important to note that the computational cost of the optimal transport problem doesn't inherently increase due to the transition to 3D itself. Rather, the cost is primarily dependent on the cardinality of the support set, which in our case corresponds to the number of degrees of freedom in the finite volume discretization. While moving to 3D typically involves a larger number of discretization points, the fundamental OT algorithms remain the same. The challenge lies in efficiently handling the increased number of degrees of freedom and potentially adapting the OT solvers to leverage the structure of 3D atmospheric data \cite{Peyre2019}. \mk{questo carino ma temo la domanda: perchè non è già stato fatto}



\section{Conclusions and Perspectives}
\label{sec:conclusions}

We presented a novel approach for reduced-order modeling of complex nonlinear dynamical systems, leveraging displacement interpolation in optimal transport theory.
Our method addresses two main challenges that are common to various scientific and engineering applications: capturing nonlinear dynamics and dealing with limited data.
By combining OT-based interpolation with POD with regression, we obtained improved accuracy and efficiency in predicting complex phenomena, as evidenced by our results on challenging benchmark problems.

The proposed framework offers several advantages over traditional ROM techniques:
i) it better captures nonlinear dynamics thanks to the OT-based interpolation;
ii) it includes an efficient data augmentation strategy that allows for improved training of deep learning-based ROMs;
iii) it improves temporal resolution through synthetic snapshot generation; iv) it is flexible in handling
nonlinear systems with limited data.

While our current results are promising, there are several avenues for future research and potential extensions of this work. One potential direction is the development of an adaptive checkpoint selection strategy to reduce the number of required checkpoints while maintaining or even improving accuracy. One could also explore advanced interpolation and extrapolation schemes to enhance the method.
Another perspective is to perform the interpolation with respect to a carefully chosen reference configuration, rather than between consecutive snapshots.
Finally, the integration of our method with real-time data assimilation techniques is another interesting research direction. By continuously updating the ROM with new observational data, one could improve long-term prediction accuracy and adapt to changing system conditions.

%The current method uses a fixed set of checkpoints for interpolation, but an adaptive approach could potentially reduce the number of required checkpoints while maintaining or even improving accuracy. This could involve using error estimators or sensitivity analysis to identify critical points in the solution trajectory where additional checkpoints would be most beneficial \cite{Peherstorfer2015}.

%Future work could explore advanced interpolation and extrapolation schemes to enhance our method. A hybrid approach that combines displacement interpolation with standard interpolation methods could offer a better trade-off between computational cost and accuracy, especially in multi-scale problems. For instance, displacement interpolation could be used for large-scale phenomena, while standard interpolation could handle smaller-scale variations \cite{Majda2003}. Additionally, the emerging concept of displacement extrapolation, which extends geodesics in the Wasserstein space beyond known data points, presents interesting possibilities for predicting system states outside the training data range.

%Another perspective is to perform the interpolation with respect to a carefully chosen reference configuration, rather than between consecutive snapshots. This approach could be particularly beneficial for periodic or quasi-periodic systems, where a single reference state might suffice for the entire simulation. The challenge here would lie in selecting an appropriate reference state and in efficiently computing the transport plans. Recent advancements in multi-marginal optimal transport could be leveraged for this purpose \cite{Pass2015}.

%The integration of our proposed method with real-time data assimilation techniques presents another significant research direction. By continuously updating the ROM with new observational data, we could improve long-term prediction accuracy and adapt to changing system conditions. This integration could be particularly valuable for various forecasting and monitoring applications, bridging the gap between model predictions and real-world observations \cite{Blum2009}.

%Finally, while our current work focuses on 2D systems, extending the method to 3D scenarios would be a natural next step. It's important to note that the computational cost of the optimal transport problem doesn't inherently increase due to the transition to 3D itself. Rather, the cost is primarily dependent on the cardinality of the support set, which in our case corresponds to the number of degrees of freedom in the discretization. While moving to 3D typically involves a larger number of discretization points, the fundamental OT algorithms remain the same. The challenge lies in efficiently handling the increased number of degrees of freedom and potentially adapting the OT solvers to leverage the structure of higher-dimensional data \cite{Peyre2019}.



==> sections/density-current.tex <==
\subsection{Density Current}
\label{subsec:density-current}
\graphicspath{{Images/density_current/}}

The density current test case simulates the evolution of a cold air bubble in a neutrally stratified atmosphere, providing a more challenging benchmark for gravity-driven flows and complex structure formation compared to the thermal bubble case.

The computational domain is $\Omega = [\SI{0}{\meter}, \SI{25600}{\meter}] \times [\SI{0}{\meter}, \SI{6400}{\meter}]$, discretized with a uniform structured mesh with mesh size of $h = \Delta x = \Delta z = \SI{100}{\meter}$, resulting in a $256 \times 64$ grid and $N_h = 16384$.
The initial conditions are:

\begin{equation}
\left\{
\begin{aligned}
{\theta}_s &= \SI{300}{\kelvin}, \\[6pt]
\theta_0 &= \begin{cases}
    {\theta}_s - \SI{7.5}{\kelvin}\left[1 + \cos(\pi r)\right] & \text{if } r \leq 1 \\
    {\theta}_s & \text{otherwise}
\end{cases} ,\\[6pt]
\rho_0 &= \frac{p_g}{R\theta_0}\left(\frac{p}{p_g}\right)^{c_v/c_p} \text{ with } p = p_g\left(1 - \frac{gz}{c_p\theta_0}\right)^{c_p/R}, \\[6pt]
\u_0 &= \mathbf{0}, \\[6pt]
\end{aligned}
\right.
\end{equation}
where $r = \sqrt{\left(\frac{x-x_c}{x_r}\right)^2 + \left(\frac{z-z_c}{z_r}\right)^2}$, with $(x_r, z_r) = (\SI{4000}{\meter}, \SI{2000}{\meter})$ and $(x_c, z_c) = (\SI{0}{\meter}, \SI{3000}{\meter})$.
We consider impenetrable, free-slip boundary conditions and run the simulation for $t_f = \SI{901}{\second}$. Figure \ref{fig:density-current-evolution} shows the evolution of the potential temperature perturbation field.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{solution_evolution.pdf}
    \caption{Evolution of the potential temperature perturbation field $\theta'$ for the density current test case.}
    \label{fig:density-current-evolution}
\end{figure}

Following \cite{Straka1993}, we set $\mu_a = \SI{75}{\meter\squared\per\second}$ and $\Pr = 1$. The reference solution uses $\Delta t_{\text{ref}} = \SI{0.005}{\second}$, while training solutions use $\Delta t_{\text{train}} \in \{\SI{0.01}{\second}, \SI{0.1}{\second}\}$. Unlike the thermal bubble case, the simulation with $\Delta t = \SI{1}{\second}$ did not converge, indicating higher sensitivity to temporal discretization.

Table \ref{tab:density_current_error} reports the discretization error, execution time, and time ratio for different training time steps. The reference FOM execution time on the test is \SI{2795.76}{\second}.

\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        $\Delta t_{\text{train}}$ & $\overline{E}_{\text{disc}}(\Delta t_{\text{train}})$ & Execution Time & Time Ratio \\
        \hline
        \SI{0.1}{\second}  & 4.40e-02 & \SI{213.04}{\second} & 13.12 \\
        \SI{0.01}{\second} & 4.76e-03 & \SI{1515.11}{\second} & 1.85 \\
        \hline
    \end{tabular}
    \caption{Discretization error $\overline{E}_{\text{disc}}(\Delta t_{\text{train}})$, execution time, and time ratio relative to the reference case (with $\Delta t = \SI{0.005}{\second}$) for different training time steps.}
    \label{tab:density_current_error}
\end{table}

Figure \ref{fig:density-current-barycenter} illustrates the evolution of synthetic solutions
for different values of $N_c$ with $\Delta t_{\text{train}} = \SI{0.1}{\second}$.
The density current evolution exhibits a combination of two distinct motion phases: a mostly vertical motion until approximately $t = \SI{280}{\second}$, followed by horizontal propagation at the ground. This dual-phase motion makes the choice of checkpoints particularly crucial for accurate interpolation, and again we see how increasing $N_c$ leads to more physically relevant interpolated trajectories.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{barycentric_field_evolution.pdf}
    \caption{Evolution of synthetic solutions for the density current as the number of checkpoints $N_c$ varies.}
    \label{fig:density-current-barycenter}
\end{figure}

Figure \ref{fig:density-current-alpha-global} shows the evolution in time of $\alpha_{\text{global}}(\cdot,\mathcal{M})$. We observe more a pronounced nonlinearity than the thermal bubble case, especially for lower values of $N_c$. This reflects the significant variations in the solution's rate of change throughout the simulation.

\begin{figure}[ht]
\centering
\includegraphics[width=1\textwidth]{alpha_global_plot.pdf}
\caption{Global interpolation parameter $\alpha_{\text{global}}(\mathcal{M})$ in red and its deviation in blue over time for $N_c = 2$ (left), $N_c = 11$ (center), $N_c = 151$ (right).}
\label{fig:density-current-alpha-global}
\end{figure}

Figure \ref{fig:density-current-generalization} presents the generalization error $E_{\text{gen}}$ for both mappings $\mathcal{M}$ and $\mathcal{L}$ and selected values of $N_c$ and $\Delta t$. Compared to the thermal bubble case, we observe higher overall error levels and more pronounced oscillations, particularly for $N_c = 2$. The difference in error magnitude between $\Delta t = \SI{0.1}{\second}$ and $\Delta t = \SI{0.01}{\second}$ is more significant, highlighting the density current's greater sensitivity to temporal discretization.
Interestingly, the errors between mapping $\mathcal{M}$ and mapping $\mathcal{L}$
are of the same order of magnitude, with only a small advantage for $\mathcal{M}$ for small $N_c$ values. This suggests that the regression task for $\alpha_{\text{global}}$ introduces an error that partially offsets the potential accuracy gain of the nonlinear mapping $\mathcal{M}$.

\begin{figure}[ht]
\centering
\includegraphics[width=1\textwidth]{generalization_error_plot.pdf}
\caption{Generalization error $E_{\text{gen}}$ over time $t$ for both mappings $\mathcal{M}$ and $\mathcal{L}$ and different values of $N_c$ and $\Delta t$. Note that the scale of the vertical
axis varies in each subplot.}
\label{fig:density-current-generalization}
\end{figure}



To further improve prediction accuracy, we implemented the POD-based correction described in Sec.~\ref{sec:ot_rom_framework}, at point (6). We collected residuals from the barycentric representation for the $\mathcal{S}_{\text{train}}$ dataset and performed POD with an energy threshold of 99.99\%. Figure \ref{fig:pod-correction} shows the effect of this correction on the mean interpolation and generalization error.
We see that the POD-based correction consistently reduces the error across different
values of $N_c$ and $\Delta t$, with the improvement being particularly significant
when using fewer checkpoints. This correction is especially valuable for capturing fine-scale structures like Kelvin-Helmholtz instability along the upper boundary of the cold front, which are challenging to represent accurately through OT-based interpolation alone.

\begin{figure}[ht]
\centering
\includegraphics[width=1\textwidth]{error_plots_mean_with_pod_corrected.pdf}
\caption{Mean interpolation error $\overline{E}_{\text{interp}}$ (left) and mean generalization error $\overline{E}_{\text{gen}}$ (right)
for both mappings $\mathcal{M}$ and $\mathcal{L}$
vs. the number of checkpoints $N_c$ for different time step sizes $\Delta t$.
The goal is to show the effect of the POD-based correction on errors $\overline{E}_{\text{interp}}$ and $\overline{E}_{\text{gen}}$.}
\label{fig:pod-correction}
\end{figure}



The effectiveness of the POD correction varies with $N_c$ and $\Delta t$. For larger time steps and fewer checkpoints, when the OT-based interpolation provides a coarser approximation, the POD correction plays a crucial role.
As $N_c$ increases or $\Delta t$ decreases, i.e., as the OT-based interpolation itself becomes more accurate, the relative impact of the POD correction diminishes.
These results demonstrate the complementary nature of OT-based interpolation and POD correction in our framework. The OT approach captures large-scale transport phenomena, while the POD correction refines the prediction by accounting for finer-scale dynamics and systematic biases. This combination allows for accurate reduced-order modeling across various temporal resolutions and checkpoint densities, making it particularly suitable for complex atmospheric flows like the density current.


==> sections/displacement-interpolation.tex <==
\section{Optimal Transport}
\label{sec:ot}

In the context of the ROM framework introduced thus far, we now turn our attention to Optimal Transport (OT) theory as a powerful tool for enhancing our approach. OT provides a mathematical foundation for interpolating between probability distributions, which we will leverage to generate synthetic snapshots and improve the representation of nonlinear dynamics in our ROM. By incorporating OT-based techniques, particularly displacement interpolation, we aim to address the challenges of capturing complex, time-dependent phenomena and enriching our dataset in scenarios where observational data may be limited. The following section introduces the key concepts of OT that form the basis of our enhanced ROM methodology.

\subsection{Foundations of Optimal Transport Theory}
OT theory \cite{Villani2008,Santambrogio2015} provides a mathematical framework to determine the most cost-effective way to transport one probability distribution into another. Below, we briefly explain that OT, in its discrete form, can be approached as a linear programming problem.

Let $\mu$ and $\nu$ be discrete measures supported on the sets $\mathcal{X} = \{x_{i}\}_{i=1}^{n}$ and $\mathcal{Y} = \{y_{j}\}_{j=1}^{m}$ and defined as follows:
\begin{equation*}
    \mu = \sum_{i=1}^n {a}_i \delta_{x_i}, \quad
    \nu = \sum_{j=1}^m {b}_j \delta_{y_j}, \quad
    \text{with} \quad \boldsymbol{a} \in \mathbb{R}_+^{n}, \quad
    \boldsymbol{b} \in \mathbb{R}_+^{m} \quad \text{s.t.} \quad
    \boldsymbol{a}^{T} \mathbf{1}_n = 1, \quad
    \boldsymbol{b}^{T} \mathbf{1}_m = 1,
\end{equation*}
where $\delta_{x_i}$ and $\delta_{y_j}$ denote Dirac delta functions at points $x_i$ and $y_j$, vectors $\boldsymbol{a}$ and $\boldsymbol{b}$ have non-negative entries representing the weights at $\{x_{i}\}_{i=1}^{n}$ and $\{y_{j}\}_{j=1}^{m}$, and $\boldsymbol{1}_{n}= [1, \ldots, 1] \in \mathbb{R}_{+}^{n}$ denotes the uniform histogram.
We define a cost function $c: \mathcal{X} \times \mathcal{Y} \rightarrow \mathbb{R}^+$, quantifying the unitary transportation cost between elements in sets $\mathcal{X}$ and $\mathcal{Y}$. This function is encapsulated in the cost matrix $\mathbf{C} \in \mathbb{R}_{+}^{n \times m}$, whose entries ${C}_{ij}$  correspond to the cost of transporting mass from $x_i$ to $y_{j}$, raised to the $p$-th power: $C_{ij} = c(x_i, y_j)^p$. The choice of $p$ depends on the specific OT problem formulation, typically $p=1$ or $p=2$.

A \textit{transport plan}\footnote{More generally, a \textit{transport plan} is a probability measure on $\mathcal{X} \times \mathcal{Y}$, whose marginals are $\mu$ and $\nu$. In discrete settings, this is typically represented by a matrix.} or \textit{coupling matrix} $\mathbf{P}$ is a matrix whose entries $P_{ij}$ encode the amount of mass transported from $x_i$ to $y_j$.
A valid transport plan must satisfy the mass conservation constraints, ensuring that the total mass sent from each $x_i$ matches the corresponding weight $a_i$, and the total mass received at each $y_j$ matches $b_j$.
The set of all feasible transport plans is given by:
\[
    \Pi(\mu, \nu) = \left\{ \mathbf{P} \in \mathbb{R}_+^{n \times m} \mid \mathbf{P} \mathbf{1}_m = \boldsymbol{a}, \ \mathbf{P}^T \mathbf{1}_n = \boldsymbol{b} \right\},
\]
and the optimal coupling $\boldsymbol{\pi} \in \Pi(\mu, \nu)$
is defined as the solution that minimizes the total transport cost:
\begin{equation}
\label{eq:unreg}
\boldsymbol{\pi} = \argmin_{\mathbf{P} \in \Pi(\mu, \nu)} \left\langle \mathbf{P}, \mathbf{C} \right\rangle,
\end{equation}
where $\langle \cdot, \cdot \rangle$ denotes the Frobenius inner product between matrices.

Problem \eqref{eq:unreg} can be solved using classical linear programming techniques \cite{transportation-simplex}. However, the computational cost of this approach can quickly become prohibitive as the size of the problems increases \cite{ot-cost}. To solve \eqref{eq:unreg} in high-dimensional settings, one can resort to entropic regularization \cite{cuturi13}, which introduces a smoothing term to the transport problem:
\begin{equation}
\boldsymbol{\pi}_{\epsilon}(\mu, \nu) = \argmin_{\mathbf{P} \in \Pi(\mu, \nu)} [\langle \mathbf{C}, \mathbf{P} \rangle - \epsilon H(\mathbf{P})] \quad \text{with} \quad H(\mathbf{P}) = -\sum_{i=1}^n \sum_{j=1}^m \mathbf{P}_{ij} (\log(\mathbf{P}_{ij})-1),
\end{equation}
where the hyperparameter $\epsilon > 0$ modulates the entropy level, making the plan more diffusive as $\epsilon$ increases. This modification leads to a differentiable and convex optimization problem that can be efficiently solved using the Sinkhorn algorithm \cite{sink}. Since this approach only involves matrix-vector multiplications, it is highly parallelizable and can take advantage of GPUs, resulting in a significant reduction of the computational cost.


\subsection{Displacement Interpolation}
\label{sub:displacement_interpolation}

Let us consider the challenge of defining interpolation between probability measures. An initial approach might be to use a convex combination of two measures $\mu_0$ and $\mu_1$, defined as:
\[
\mu_\alpha = (1-\alpha) \mu_0 + \alpha \mu_1, \quad \alpha \in [0,1] .
\]
However, this linear interpolation is counterintuitive in the context of OT problems because it simply redistributes the mass across the supports of measures $\mu_0$ and $\mu_1$ based on the interpolation parameter $\alpha$, rather than actually transporting mass from one measure to another. Ideally, we would prefer the mass to transition smoothly, effectively moving between the supports.

In the scenario involving Dirac delta measures, a desirable interpolation is given by their McCann interpolation \cite{mccan-interpolation}:
\begin{equation}
    \label{eq:di-deltas}
\mu_\alpha = \delta_{(1-\alpha)x_0 + \alpha x_1} \quad \alpha \in [0,1];
\end{equation}
where $x_0$ and $x_1$ are the locations of the original Dirac deltas.

To extend this approach to discrete distributions, consider two discrete probability measures $\mu_0 = \sum_{i=1}^n a_i \delta_{x_i}$ and $\mu_1 = \sum_{j=1}^m b_j \delta_{y_j}$ supported on the same metric space $(\mathcal{X}, d)$. Let $\boldsymbol{\pi} \in \Pi(\mu_0, \mu_1)$ be the OT plan between $\mu_0$ and $\mu_1$, obtained by solving \eqref{eq:unreg}. Then, a generalization of \eqref{eq:di-deltas} is as follows:
\begin{equation}
\label{eq:disp-int}
\mu_\alpha = \sum_{i,j} \pi_{i,j} \delta_{(1-\alpha)x_i + \alpha y_j}  \quad \alpha \in [0,1].
\end{equation}
This interpolation method, known as \textit{displacement interpolation}\footnote{In the most general continuous case, the displacement interpolation is $\mu_\alpha = (e_\alpha)_\# \pi$ where $e_\alpha: \mathcal{X} \times \mathcal{X} \to \mathcal{X}$ is the evaluation map $e_t(x,y) = (1-\alpha)x + ty$, and $(e_\alpha)_\#$ denotes the push-forward operation.}, plays a fundamental role in the field of optimal transport, particularly with regard to the time-dependent version of OT (\cite[Ch.~5]{villani2021topics}). In the discrete-to-discrete setting, this method has an intuitive geometric interpretation: each particle of mass from $\mu_0$ moves towards $\mu_1$ according to the optimal transport plan, taking straight-line paths to their final destinations. See Figure \ref{fig:optimal_transport_di} for an example. At the specified parameter $\alpha$, $\mu_\alpha$ represents the distribution of all particles at their intermediate positions\footnote{In our framework, $\alpha$ is treated as a virtual time parameter, distinct from the physical time $t$. This allows us to interpolate between distributions using $\alpha$ while maintaining a separate notion of actual time evolution in the system.}.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{displacement_interpolation.pdf}
    \caption{Displacement interpolation between two discrete distributions $\mu_0$ and $\mu_1$ shown on the left panel. In the right panel, the point's masses are proportional to the size of the point and OT plan line thickness are proportional to the mass transported.}
    \label{fig:optimal_transport_di}
\end{figure}

Key properties of displacement interpolation include: (i) geodesicity, as $\mu_\alpha$ traces a geodesic in the Wasserstein space of probability measures; (ii) mass conservation with $\mu_\alpha(X) = 1$ for all $\alpha$; and (iii) finite support at each $\alpha$, accommodating at most $nm$ support points. To the readers interested in more details on displacement interpolation and its properties, we recommend the seminal work by McCann \cite{mccan-interpolation} and the in-depth discussions in Santambrogio's book \cite{Santambrogio2015}, particularly Chapter 5.


==> sections/everything.tex <==
\section{OT-based DL-framework}\label{sec:complete_framework}
In this section, we exploit the methodologies discussed in the previous sections to introduce the optimal transport based model order reduction approach we developed, which takes advantage of the Sinkhorn divergence kernel for the kPOD and of a neural network regression for the backward map problem.

\subsection{Sinkhorn Kernel}
% For our study, we have investigated the use of a kernel based on the Sinkhorn divergence.
Let $\mathcal{X} = \{x_{i}\}_{i = 1}^{N_{h}}$ be a set of discrete input data, and $\mu, \nu$ be two probability measures over $\mathcal{X}$, represented by the two probability mass functions $f,g:\mathcal{X} \to [0,1]$.

The kernel we propose for the kPOD is given by:
\begin{equation}
    \label{eq:sink-kern}
\kappa( \mu, \nu) = \left[\frac{1}{2} \sum_{i=1}^{N_{h}} {x_{i}}^{T} {x_{i}} f({x_{i}}) +
\frac{1}{2} \sum_{j=1}^{N_{h}} {y_{j}}^{T} {y_{j}} g({y_{j}}) \right]
-S_{\epsilon}(\mu,\nu),
\end{equation}
where $x_{i}$ and $y_{j}$ denote the support points of $\mu$ and $\nu$ respectively, and $S_{\epsilon}(\mu,\nu)$ can be efficiently computed using the Sinkhorn-Knopp algorithm (see Section \ref{sec:ot}).
The motivation behind this formula is to obtain a weighted version of the $l^{2}$ discrete product that takes into account the transport plan.

Considering the regularity of Monge's Problem, we ensure that an optimal transport map $T:\mathcal{X} \to \mathcal{X}$ exists, and it is bijective. Consequently, the inverse map $T^{-1}:\mathcal{X} \to \mathcal{X}$ also exists, leading to the relationships ${x}_{i} = T^{-1}({y}_{i})$ and ${y}_{i} = T({x}_{i})$. Here, the set $\left\{y_{i}\right\}_{i = 1}^{N_{h}}$ represents a proper permutation of $\left\{x_{i}\right\}_{i = 1}^{N_{h}}$ which solves the Monge's Problem.


Exploiting these properties, one can easily rewrite the bivariate symmetric form as:

\begin{equation}
    \label{kernel_form2}
\kappa(\mu, \nu) = \sum_{i=1}^{N_{h}} {x_{i}}^{T} T({x_{i}}) f({x_{i}}) =
\sum_{i=1}^{N_{h}} {y_{i}}^{T} T^{-1}({y_{i}}) g({y_{i}}) = \kappa (\nu, \mu) .
\end{equation}
To prove the equivalence between Equations \eqref{eq:sink-kern} and \eqref{kernel_form2}, we start by considering the case of computing $\kappa(\mu,\mu)$. In this scenario, the optimal transport map is equal to the identity, denoted as $\mathcal{I}:\mathcal{X} \to \mathcal{X}$. Consequently, we have:

\begin{equation}
\kappa(\mu, \mu) = \sum_{i = 1}^{N_{h}} {x_{i}}^{T} \mathcal{I}({x_{i}}) f({x_{i}}) =
\sum_{i = 1}^{N_{h}} {x_{i}}^{T} {x_{i}} f({x_{i}}).
\end{equation}
This reduces the kernel $\kappa(\mu, \mu)$ to the second moment of the probability distribution $\mu$.

Next, we develop the Wasserstein distance in the quadratic cost case:
%\todofp{ricontrolla anche qui}
\begin{equation}
    W_{2}^{2}(\mu,\nu) = \sum _{ i = 1 }^{N_{h}}   \mid{x_{i}} - T({x_{i}})\mid^{2} f({x_{i}}) = \sum _{i =1 }^{N_{h}}( {x}_{i}^{T} {x_{i}} + T({x}_{i})^{T} T({x}_{i}) - 2 {x_{i}}^{T}T({x}_{i})) f({x}_{i}).
\end{equation}
After isolating the mixed product term, which corresponds to the kernel $\kappa(\mu,\nu)$, we can use the pushback $T_{\#} \mu= \nu$ to obtain:
\begin{equation}
\kappa( \mu, \nu) = \left[\frac{1}{2} \sum_{i=1}^{N_{h}} {x_{i}}^{T} {x_{i}} f({x_{i}}) +
\frac{1}{2} \sum_{j=1}^{N_{h}} {y_{i}}^{T} {y_{i}} g({y_{i}})\right]
-W_{2}^{2}(\mu,\nu) .
\end{equation}
Our approach aims to utilize the Sinkhorn divergence as an approximation for the $W_2^{2}(\cdot,\cdot)$ distance, thereby defining the kernel presented in Equation \eqref{eq:sink-kern}. As shown, this kernel is equivalent to the one presented in Equation \eqref{kernel_form2}, but it eliminates the need for an explicit computation of the optimal transport map $T$.

\begin{remark}
Consider a possible extension of the Gaussian kernel, where we replace the Euclidean distance with the Sinkhorn divergence:

\begin{equation}
\kappa( \mu, \nu) = \exp\left(-\frac{1}{\sigma} (S_{\epsilon}(\mu,\nu))^{2}\right),
\end{equation}
and the parameter $\sigma$ controls the smoothness of the kernel.
It can be proved that this kernel, known as the Wasserstein exponential kernel \cite{Plaen2020}, lead to a Gram matrix representing a first-order approximation of the kernel we propose, up to a rank-one matrix.
\end{remark}



\subsection{Neural network architectures}
To construct the backward map, we employ a neural network regression approach to learn the mapping between the reduced-order coefficients and the full-order solution, which corresponds to the inverse mapping of kPOD. We explore two distinct neural network architectures for this purpose: a decoder-only architecture and a complete autoencoder architecture.

\subsubsection{Decoder-based approach}

In the decoder-only architecture, we construct a neural network that takes the kPOD coefficients $\boldsymbol{z} \in \mathbb{R}^{k}$ as input and generates the full-order solution $\boldsymbol{u}^{D}_{\text{NN}} \in \mathbb{R}^{N_{h}}$ as output.

The decoder function $\psi^{D}(\boldsymbol{z};{\Theta}^{D})$ is defined by a set of weights and biases ${\Theta^{D}}$, which are learned during the training process. Once trained, it can be used to evaluate the backward mapping as:

\begin{equation}
      \boldsymbol{u}^{D}_{\text{NN}} = f^{D}(\boldsymbol{z};{\hat{\Theta}}^{D}) \approx F^{-1}(\boldsymbol{z}) .
\end{equation}
To find the optimal parameter vector $\hat{\Theta}^{D}$, we employ a supervised learning paradigm that involves optimizing a properly selected loss function $\mathcal{J}^{D}$:

\begin{equation}
\label{nn-opt}
{\hat{\Theta}^{D}}=\underset{{\Theta}^{D}}{\operatorname{argmin}} \ \mathcal{J}^{D}({\Theta}^{D}),
\end{equation}
which measures the discrepancy between the true full-order solutions and the output of the neural network. The optimization process aims to minimize this discrepancy by adjusting the parameters ${\Theta}^{D}$, leading to an accurate decoder model that can effectively reconstruct the full-order solutions from the kPOD coefficients.


\subsubsection{Autoencoder-based approach}

In the complete autoencoder architecture, we extend the decoder-based approach by adding an encoder component to the neural network.
The encoder function $\psi^{E}(\cdot;{\Theta^{E}})$ is parameterized by the set of weights and biases ${\Theta^{E}}$, and it maps the full-order solution to the kPOD reduced order coefficients:

\begin{equation}
    \boldsymbol{z}^{\text{AE}}_{\text{NN}} =  \psi^{E}(\boldsymbol{u}_{h};{\Theta^{E}}).
\end{equation}
The decoder function $\psi^{D}(\cdot;{\Theta^{D}})$ is the same as in the decoder-based approach, and it maps the reduced order coefficients back to the full-order solution:

\begin{equation}
    \boldsymbol{u}^{\text{AE}}_{\text{NN}} = \psi^{D}(\boldsymbol{z}^{\text{AE}}_{\text{NN}};{\Theta^{D}}).
\end{equation}
During the learning procedure we seek the optimal configuration of the encoder and decoder weights such that we can approximate the forward and backward mapping as follows:

\begin{equation}
    \left\{\begin{aligned}
            &\psi^E(\boldsymbol{u}_h ; \hat{\Theta}^E)\approx F(\boldsymbol{u}_h), \\
            &\psi^D(\boldsymbol{z}^{\text{AE}}_{\text{NN}} ; \hat{\Theta}^D) \approx F^{-1}(\boldsymbol{z}^{\text{AE}}_{\text{NN}}).
        \end{aligned} \right.
\end{equation}
To find the optimal weights $(\hat{\Theta}^{E},\hat{\Theta}^{D})$, we minimize the joint loss function defined as:

\begin{equation}
\label{ae-opt}
(\hat{\Theta}^{E},\hat{\Theta}^{D})=\underset{(\Theta^{E},\Theta^{D})}{\operatorname{argmin}} \ \mathcal{J}^{I_d}(\Theta^{E},\Theta^{D})+ \lambda \mathcal{J}^{\text{kPOD}}(\Theta^{E}).
\end{equation}
The first term, namely $\mathcal{J}^{I_{d}}$, is the reconstruction loss and measures the difference between the input and output of the autoencoder.
On the other hand, $\mathcal{J}^{\text{kPOD}}$ represents the kPOD loss, and measures the discrepancy between the encoded coefficients and the true kPOD coefficients obtained using Equation \eqref{forward-map}.
The hyperparameter $\lambda \in \mathbb{R}_{+}$ plays a crucial role in balancing the contributions of these two terms during training. It allows us to control the trade-off between the reconstruction accuracy and the faithfulness of the reduced order representation.

\subsection{Neural Network Training}
\label{subsec:training}

The neural network regression in our implementation is performed using two types of architectures: feedforward and convolutional layers.
% These architectures are evaluated for test cases involving scalar fields defined on 2D domains and discretized on structured meshes, which can be treated as single-channel images.
The characteristics of these architectures are presented in Appendix \ref{app:arch}.

To obtain the optimal parameters, we employ a supervised learning paradigm. Specifically, we have $N_{\text{tr}}$ pairs of full-order solutions and their corresponding kPOD coefficients $\{(\boldsymbol{u}_{h}^{i},\boldsymbol{z}^{i})\}_{i=1}^{N_{\text{tr}}}$. During each epoch, we iterate over the training data and calculate the reconstruction loss, which can be chosen either as the Mean Squared Error (MSE) or the Sinkhorn divergence.

When using the MSE measure, the general loss term can be written as:
\begin{equation}
    \mathcal{J}(\Theta) = \frac{1}{N_{\text{tr}}} \sum_{i=1}^{N_{\text{tr}}} \|\boldsymbol{y}^{i} - \boldsymbol{y}_{\text{NN}}^{i}(\Theta)\|^{2},
\end{equation}
where the expressions for the NN output $\boldsymbol{y}_{\text{NN}}(\Theta)$ and the desired output $\boldsymbol{y}$ need to be specialized depending on the type of network under consideration, as shown in Table \ref{tab:loss-function-comparison}.

On the other hand, when using the Sinkhorn divergence, each sample is treated as a point belonging to the support of a probability distribution. Therefore, we have the following expressions for the distribution produced by the network $\nu_{\text{NN}}$ and the desired distribution $\mu$:

\begin{equation}
    \mu = \frac{1}{N_{\text{tr}}} \sum_{i=1}^{N_{\text{tr}}} \delta_{\boldsymbol{y}^{i}}, \quad \nu_{\text{NN}} = \frac{1}{N_{\text{tr}}} \sum_{j=1}^{N_{\text{tr}}} \delta_{\boldsymbol{y}_{\text{NN}}^{j}(\Theta)} \, .
\end{equation}
These distributions allow us to calculate the loss function as the Sinkhorn divergence by means of:

\begin{equation}
    \mathcal{J}(\Theta) = S_{\epsilon}(\mu, \nu_{\text{NN}}).
\end{equation}
In this case, to ensure the correct coupling of the input and output distributions while preserving their order, an initial training phase using the MSE loss for a limited number of epochs is required.
To prevent overfitting, we implement an early stopping criterion, and we set the total number of epochs to $10^3$.

The neural network architectures are implemented using PyTorch \cite{pytorch}, while the Sinkhorn divergence is computed using the geomLoss package \cite{feydy2019interpolating}.
The experiments are conducted on a machine equipped with an NVIDIA GeForce RTX 3080 GPU and an 11th Gen Intel(R) Core(TM) i7-11700 @ 2.50GHz processor running CentOS Stream release 8.

\renewcommand{\arraystretch}{1.5}
\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        \cellcolor[HTML]{E5E3E3}Loss Function & \cellcolor[HTML]{E5E3E3}$\boldsymbol{y}$ & \cellcolor[HTML]{E5E3E3}$\boldsymbol{y}_{\text{NN}}$ \\
        \hline
                    $\mathcal{J}^D$ & \ $\boldsymbol{u}_{h}$ \ & \ $\boldsymbol{u}_{\text{NN}}^D$ \ \\
                      $\mathcal{J}^{I_d}$ & $\boldsymbol{u}_{h}$ & $\boldsymbol{u}_{\text{NN}}^{\text{AE}}$ \\
                      $\mathcal{J}^{\text{kPOD}}$ & $\boldsymbol{z}$ & $\boldsymbol{z}_{\text{NN}}^{\text{AE}}$ \\
        \hline
    \end{tabular}
    \caption{Comparison of Loss Functions and Outputs.}
    \label{tab:loss-function-comparison}
\end{table}


==> sections/fom_model.tex <==
\section{Problem Definition and Its Numerical Discretization}\label{sec:FOM}

If we neglect the effects of moisture, solar radiation, and ground heat flux, the dynamics of the dry atmosphere can be described by the Euler equations:
\begin{align}
&\frac{\partial \rho}{\partial t} + \nabla \cdot (\rho \u) = 0 &&\text{in} \ \Omega \ \times \ (0, t_f], \label{eq:continuity} \\
&\frac{\partial (\rho \u)}{\partial t} + \nabla \cdot (\rho \u \otimes \u) + \nabla p + \rho g \widehat{\mathbf{k}} = \mathbf{0} &&\text{in} \ \Omega \ \times \ (0, t_f], \label{eq:momentu} \\
&\frac{\partial (\rho e)}{\partial t} + \nabla \cdot (\rho \u e) + \nabla \cdot (p \u) = 0 &&\text{in} \ \Omega \ \times \ (0, t_f].\label{eq:energy}
\end{align}
where the unknowns are the air density $\rho$, the wind velocity $\u$, the pressure $p$, and the total energy density $e$, which is defined as:
\begin{equation}
e = c_v T + \frac{1}{2}|\u|^2 + gz, \label{eq:total_energy_density}
\end{equation}
where $T$ is the temperature and $c_v=715.5$ J/(Kg K) is the specific heat capacity at constant volume. Additionally, $g$ is the gravitational constant and $\widehat{\mathbf{k}}$ is the unit vector in the vertical $z$ direction. Eqs.~\eqref{eq:continuity}-\eqref{eq:energy} state conservation of mass, momentum, and total energy, respectively.
We assume that dry air behaves as an ideal gas \cite{Pielke2002}. Then, for closure we add to  system \eqref{eq:continuity}-\eqref{eq:energy} the ideal gas law:
\begin{align}
p = \rho R T \quad \text{in} \ \Omega \ \times \ (0, t_f], \label{eq:EQ_of_State}
\end{align}
where $R= 287$ J/(Kg K) is the specific gas constant for dry air.

For numerical stability, we add an artificial diffusion term to the momentum and energy equations:
\begin{align}
&\frac{\partial (\rho \u)}{\partial t} +  \nabla \cdot (\rho \u \otimes \u) + \nabla p + \rho g \widehat{\mathbf{k}}  - \mu_a \Delta \u = \mathbf{0}  &&\text{in } \Omega \times (0,t_f], \label{eq:momentum_stab}\\
&\frac{\partial (\rho e)}{\partial t} +  \nabla \cdot (\rho \u e) +   \nabla \cdot (p \u) - c_p \dfrac{\mu_a}{Pr} \Delta T = 0 &&\text{in } \Omega \times (0,t_f], \label{eq:energy_stab}
\end{align}
where $\mu_a$ is a constant (artificial) diffusivity coefficient and $Pr$ is the Prandtl number. We note that this is equivalent to using a basic eddy viscosity model in Large Eddy Simulation (LES) \cite{BIL05}. More sophisticated LES models can be found in, e.g., \cite{CGQR, marrasNazarovGiraldo2015}.

It is typical to decompose the pressure into a  baseline state $p_0$, coinciding with the pressure in hydrostatic balance, and a perturbation $p^{\prime}$:
\begin{align}
p = p_0 + p'. \label{eq:EQ_p_splitting}
\end{align}
We can apply a similar decomposition to the density:
\begin{align}
\rho = \rho_0 + \rho'. \label{eq:rhoPrime}
\end{align}
Note that from eq. \eqref{eq:EQ_of_State} we have:
\begin{align}
\rho_0 = \dfrac{p_0}{R T_0}.
\label{eq:rho_hyd}
\end{align}
and the assumption of hydrostatic balance gives:
\begin{align}
\nabla p_0 + \rho_0 g \widehat{\mathbf{k}} = \boldsymbol{0}. % = - \dfrac{p_0}{R T_0} g \widehat{\bk},
\label{eq:p0_hydro}
\end{align}
By plugging \eqref{eq:EQ_p_splitting} into \eqref{eq:momentum_stab} and  accounting for \eqref{eq:rho_hyd}, we can recast the momentum conservation equation into:
\begin{align}
&\frac{\partial (\rho \u)}{\partial t} +  \nabla \cdot (\rho \u \otimes \u) + \nabla p' + \rho' g \widehat{\mathbf{k}} - \mu_a \Delta \u = \mathbf{0}  &&\text{in } \Omega \times (0,t_f]. \label{eq:momeCE2}%\label{eq:energyCE2}
\end{align}
Concerning eq.~\eqref{eq:energy_stab}, it is worth noting that a quantity of interest for atmospheric problems is the potential temperature
\begin{equation}
\label{eq:potential_temperature}
\theta = \frac{T}{\pi}, \quad \pi = \left( \frac{p}{p_g} \right)^{\frac{R}{c_p}},
\end{equation}
where $\pi$ is the so-called Exner pressure, $p_g = 10^5$ Pa is standard pressure at the ground, and $c_p = c_v + R$ is the specific heat capacity at constant pressure for dry air.
In order to avoid computing \(\theta\) in a post-processing phase, one can replace eq.~\eqref{eq:energy_stab} with:
\begin{equation}
\label{eq:energy3}
\frac{\partial (\rho \theta)}{\partial t} + \nabla \cdot (\rho \u \theta)  - \dfrac{\mu_a}{Pr} \Delta \theta
= 0 \quad \text{in} \ \Omega \ \times \ (0, t_f].
\end{equation}
Equation of state \eqref{eq:EQ_of_State} in terms of $\theta$ instead of $T$ is:
\begin{equation}
\label{eq:state_potential}
p = p_g \left( \frac{\rho R \theta}{p_g} \right)^{\frac{c_p}{c_v}}.
\end{equation}
The use of potential temperature offers several advantages, especially for adiabatic atmospheric processes. For instance, in adiabatic hydrostatic conditions, the potential temperature remains constant with respect to the height from the ground and equal to the absolute atmospheric temperature at the ground level.

The system to be solved is given by eqs.~\eqref{eq:continuity}, \eqref{eq:EQ_p_splitting}, \eqref{eq:rhoPrime}, \eqref{eq:momeCE2}, \eqref{eq:energy3} and \eqref{eq:state_potential}, which needs to be supplemented with appropriate initial and boundary conditions.
For more details on the formulation of the Euler equations adopted in this work and a comparison of different formulations, we refer the interested reader to, e.g.,  \cite{girfoglio2024comparative}.
In order to efficiently solve the coupled problem, we adopt a splitting approach thoroughly described in \cite{Girfoglio_2023, girfoglio2024comparative, CGQR}, which uses Backward Differencing Formula of first order (BDF1) for the approximation of the time derivative, a semi-implicit scheme for the convective terms,  a fully implicit method for the diffusion terms, and a second-order Finite Volume method for space discretization.

For more details about the numerical method, the reader is referred to \cite{Girfoglio_2023,girfoglio2024comparative,CGQR}.


==> sections/framework.tex <==
\section{OT-Based Interpolation ROM}
\label{sec:ot_rom_framework}

We now present a comprehensive framework for reduced order modeling leveraging displacement interpolation.
This approach combines the theoretical foundations of OT with practical strategies for data extension and efficient online inference, particularly suited for problems with complex, nonlinear dynamics, such as convection-dominated flows described by the model in Sec.~\ref{sec:FOM}.

Let $\mathcal{S}_h = \{\boldsymbol{u}_{h}^{k}=\boldsymbol{u}_{h}(t_{k})\}_{k=0}^{N_{T}-1} \subset \mathbb{R}^{N_{h}}$ be the discretized trajectory set of the FOM solution, as defined in Sec.~\ref{sec:rom-model}.
Our framework aims to extend this discrete set into a continuous representation using OT-based interpolation.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Images/scheme.pdf}
    \caption{Schematic depiction of our OT-based interpolation ROM approach.}
    \label{fig:scheme}
\end{figure}

Our methodology, depicted in Figure \ref{fig:scheme}, can be subdivided in the following key steps:

\begin{enumerate}
\setlength\itemsep{1em}
\item \textbf{Checkpoint Selection:} we select a subset of $N_c$ checkpoints from $\mathcal{S}_h$, denoted as $\mathcal{C} = \{\boldsymbol{u}_{h}^{k_i}\}_{i=0}^{N_c-1}$, where $0 = k_0 < k_1 < \cdots < k_{N_{c-1}} = N_T -1$. The number of checkpoints $N_c$ is a parameter of the method, allowing for a trade-off between accuracy and computational
efficiency.

\item \textbf{Displacement Interpolation:} for each pair of consecutive checkpoints $(\boldsymbol{u}_{h}^{k_i}, \boldsymbol{u}_{h}^{k_{i+1}})$, we solve the entropic regularized OT problem as described in Sec.~\ref{sub:displacement_interpolation}:
\begin{equation}
    \label{eq:step2}
    \boldsymbol{\pi}_{\epsilon}(\mu_i, \mu_{i+1}) = \argmin_{\mathbf{P} \in \Pi(\mu_i, \mu_{i+1})} [\langle \mathbf{C}, \mathbf{P} \rangle - \epsilon H(\mathbf{P})],
\end{equation}
where $\mu_i$ and $\mu_{i+1}$ are the probability measures corresponding to $\boldsymbol{u}_{h}^{k_i}$ and $\boldsymbol{u}_{h}^{k_{i+1}}$ respectively, and $\epsilon > 0$ is the entropic regularization parameter. For scalar fields, we employ one of two strategies: (i) if the field is non-negative, we normalize it to have unit mass, or (ii) we split the field into positive and negative components, normalizing each separately, and perform the procedure for both.

\item \textbf{Synthetic Data Generation:} Let $\mathcal{X} =\{x_l\}_{l=1}^{N_h}$ be the set of discretization points in our numerical scheme, shared by all fields. These points represent, for example, cell centroids in a FV discretization.
Let $\alpha \in [0,1]$ be the local interpolation parameter, playing the role of virtual time. We define a function $\boldsymbol{u}_{\text{synth}}(i,\alpha)$, for $i \in \{0, 1, \ldots, N_c-2\}$, that generates synthetic snapshots using the OT plan $\boldsymbol{\pi}_{\epsilon}$:
\begin{equation}
    \label{eq:u_synth}
    \boldsymbol{u}_{\text{synth}}(i,\alpha) = \underbrace{\left((1-\alpha)\|\boldsymbol{u}_h^{k_i}\|_1 + \alpha\|\boldsymbol{u}_h^{k_{i+1}}\|_1\right)}_{\text{(A)}} \sum_{l,m} (\boldsymbol{\pi}_{\epsilon})_{lm} \delta_{\text{proj}_{\mathcal{X}}((1-\alpha)x_l + \alpha x_m)},
\end{equation}
where $\|\cdot\|_1$ denotes the L1 norm.
In \eqref{eq:u_synth}, term (A)
interpolates the total mass between consecutive checkpoints and the function $\text{proj}_{\mathcal{X}}(\cdot)$ maps a point to the nearest point in $\mathcal{X}$, ensuring that the interpolated value is associated with the correct discretization point in our numerical scheme\footnote{In our FV implementation, $\text{proj}_{\mathcal{X}}(\cdot)$ specifically maps a point to the centroid of its containing cell. This ensures that the interpolated value is correctly associated with the cell-averaged quantities typical in FV discretizations.}.

We generate a set of $N_{\text{synth}}$ synthetic snapshots within each interval $[t_{k_i}, t_{k_{i+1}}]$:
\begin{equation}
    \boldsymbol{u}_{\text{synth}}^{i,j} = \boldsymbol{u}_{\text{synth}}(i, \alpha_j), \quad \text{where} \quad \alpha_j = j/(N_{\text{synth}}+1) \quad \text{for} \quad j = 1, \ldots, N_{\text{synth}}.
\end{equation}
These synthetic snapshots enrich our dataset, providing a denser sampling of the solution manifold for the time-interpolation parameter mapping and the subsequent POD step, which captures the dominant modes of the system's behavior.


\item \textbf{Time-Interpolation Parameter Mapping:} We seek a mapping between the physical time $t$ and the interpolation parameter $\alpha$, to label the synthetic snapshots with ``real'' instead of ``virtual'' time. To better understand this concept, we define $\alpha_{\text{local}} \in [0,1]$ as the interpolation parameter within a specific interval between two checkpoints, and $\alpha_{\text{global}} \in [0,1]$ as the overall progress through the entire simulation.
For equispaced checkpoints with interval $\Delta t_c = \frac{t_f}{N_c - 1}$, we express $\alpha_{\text{global}}$ as:
\begin{equation}
\alpha_{\text{global}} = \frac{i\Delta t_c}{t_f} + \alpha_{\text{local}}\frac{\Delta t_c}{t_f} = \frac{i + \alpha_{\text{local}}}{N_c - 1}, \quad i \in \{0, 1, ..., N_c - 2\},
\end{equation}
where $i$ is the index of the current checkpoint interval. The first term represents the fraction of the total real time that has elapsed up to the start of the current checkpoint interval, while the second term represents the progress within the current interval.

We aim to find a mapping $\mathcal{F} = (\mathcal{F}_1,\mathcal{F}_2): [0, t_f] \rightarrow \{0,\ldots,N_c-2\} \times [0, 1]$ that returns the interval index $i$ and the local interpolation parameter $\alpha_{\text{local}}$ for any given time $t$. We propose two strategies:
\begin{itemize}
    \item[-] \textbf{Linear Mapping:} We define a piecewise linear mapping $\mathcal{L}: [0, t_f] \rightarrow \{0,\ldots,N_c-2\} \times [0, 1]$ as:
\begin{equation}
    \mathcal{L}(t) = \left(\left\lfloor\frac{t}{\Delta t_c}\right\rfloor,\ \frac{t - t_{k_i}}{t_{k_{i+1}} - t_{k_i}}\right), \quad t \in [t_{k_i}, t_{k_{i+1}}],
\end{equation}
assuming a uniform progression of $\alpha_{\text{local}}$ with respect to time within each checkpoint interval and set $\mathcal{F} = \mathcal{L}$.
\item[-] \textbf{MinL2 Regression:} We find the optimal mapping $\mathcal{M}: [0, t_f] \rightarrow \{0,\ldots,N_c-2\} \times [0, 1]$ by solving:
\begin{equation}
\label{eq:minL2}
    \mathcal{M}(t) = \argmin_{(g_1, g_2)} \sum_{k=0}^{N_T} \|\boldsymbol{u}_h^k - \boldsymbol{u}_{\text{synth}}(g_1(t_k), g_2(t_k))\|_2^2,
\end{equation}
where $g_1: [0, t_f] \rightarrow \{0,\ldots,N_c-2\}$ determines the interval index and $g_2: [0, t_f] \rightarrow [0, 1]$ determines the local interpolation parameter. In practice, we solve problem \eqref{eq:minL2} using a dictionary-based approach.
First, for each discrete time point $t_k$, we compute:
\begin{equation}
\alpha_{\text{global},k} =  \frac{i^* + j^*/(N_{\text{synth}}+1)}{N_c -1}, \quad (i^*, j^*) = \argmin_{(i,j)} ||\boldsymbol{u}_h(t_k) - \boldsymbol{u}_{\text{synth}}^{i,j}||_2^2.
\end{equation}
Then, we perform a regression on the resulting database $\{(t_k, \alpha_{\text{global},k})\}_{k=0}^{N_T-1}$ to obtain a continuous function $\tilde{\alpha}_{\text{global}}: [0, t_f] \rightarrow [0, 1]$.
For any given time $t$, we can compute the interval index $\tilde{i}$ and local interpolation parameter $\tilde{\alpha}_{\text{local}}$ from the predicted $\tilde{\alpha}_{\text{global}}(t)$ as follows:
\begin{equation}
\begin{aligned}
    \tilde{i} &= \lfloor \tilde{\alpha}_{\text{global}}(t) \cdot (N_c - 1) \rfloor, \quad \text{and} \quad   \tilde{\alpha}_{\text{local}} &= \tilde{\alpha}_{\text{global}}(t) \cdot (N_c - 1) - \tilde{i},
\end{aligned}
\end{equation}
expressing the MinL2 regression mapping as $\mathcal{M}(t) = (\tilde{i}, \tilde{\alpha}_{\text{local}})$. Then, we set $\mathcal{F} = \mathcal{M}$.
\end{itemize}

\item \textbf{Online Inference:} For a given time $t^*$, we predict the solution $\boldsymbol{u}_h(t^*)$ using the chosen mapping $\mathcal{F}$:
\begin{equation}
    \label{eq:online_inference}
    \boldsymbol{u}_h(t^*) \approx \boldsymbol{u}_{\text{synth}}(\mathcal{F}_1(t^*), \mathcal{F}_2(t^*)),
\end{equation}
where $\mathcal{F}_1$ and $\mathcal{F}_2$ are the components of $\mathcal{F}$. This step allows for rapid prediction of system states at arbitrary time points, leveraging the pre-computed OT plans and time-$\alpha$ mappings.
\item \textbf{POD-based Correction:} To enhance prediction accuracy, we introduce a correction step based on POD with regression (POD-R) of the residuals. Let $\mathbf{R} = [\boldsymbol{r}_0 | \cdots | \boldsymbol{r}_{N_T-1}] \in \mathbb{R}^{N_h \times N_T}$ be the matrix of residuals, where $\boldsymbol{r}_k = \boldsymbol{u}_h^k - \boldsymbol{u}_{\text{synth}}(\mathcal{F}_1(t_k), \mathcal{F}_2(t_k))$ for $k = 0, \ldots, N_T-1$. We perform POD on $\mathbf{R}$ to obtain a reduced basis $\mathbf{U}_r \in \mathbb{R}^{N_h \times N_r}$. The columns of $\mathbf{U}_r$ form a basis for the dominant modes of the residuals, capturing systematic biases in the OT-based interpolation.

We train a Gaussian Process Regression (GPR) model $\mathcal{G}: [0, t_f] \rightarrow \mathbb{R}^{N_r}$ to predict the POD coefficients of the residuals:
\begin{equation}
    \delta \boldsymbol{\alpha}_r(t) = \mathcal{G}(t),
\end{equation}
where $\delta \boldsymbol{\alpha}_r(t)$ are the POD coefficients of the residual at time $t$. Then, the corrected prediction for $\boldsymbol{u}_h(t^*)$ is given by:
\begin{equation}
    \label{eq:corrected_prediction}
    \boldsymbol{u}_h(t^*) \approx \boldsymbol{u}_{\text{synth}}(\mathcal{F}_1(t^*), \mathcal{F}_2(t^*)) + \mathbf{U}_r \delta \boldsymbol{\alpha}_r(t^*).
\end{equation}
This correction compensates for the bias in the barycentric representation, improving the alignment with the true solution manifold.
\end{enumerate}


\begin{rem}
\label{remark1}
It is worth noting that, for each checkpoint, $\alpha_{\text{local}}$ is either 0 (at the start of an interval) or 1 (at the end of an interval). Therefore, the corresponding $(t,\alpha_{\text{global}})$ pairs at the checkpoints can be expressed as:
\begin{equation}
\left(t_{k_i}, \alpha_{\text{global}}(t_{k_i})\right) = \left(i \Delta t_c, \frac{i}{N_c - 1}\right), \quad 0 \le i \le N_c -1,
\end{equation}
where $i$ represents the checkpoint index. These points form a diagonal line in the $[0,t_f] \times [0,1]$ space.
\end{rem}

\begin{rem}
\label{remark2}
As $N_c$ increases, $\alpha_{\text{global}}(\cdot,\mathcal{M})$ converges towards $\alpha_{\text{global}}(\cdot,\mathcal{L})$. This is due to the increased density of fixed points where both mappings must agree, reducing the scope for $\mathcal{M}$ to deviate from $\mathcal{L}$ between checkpoints. Consequently, local nonlinearities captured by $\mathcal{M}$ become negligible compared to the overall linear trend.
\end{rem}

While the complete framework provides a comprehensive ROM model, the initial steps (1)-(3)
alone provide a \emph{data augmentation} technique
that can be valuable for the training of different
non-intrusive ROMs.
The synthetic data generation process allows us to construct a comprehensive snapshot matrix that captures both the original checkpoints and the interpolated states. We define this synthetic snapshot matrix $\mathbf{S}_{\text{synth}} \in \mathbb{R}^{N_h \times N_\text{tot}}$, where $N_\text{tot} = N_\text{synth}(N_c - 1) + N_c $ is the total number of snapshots including the checkpoints:
\begin{equation}
    \mathbf{S}_{\text{synth}} = [\boldsymbol{u}_{h}^{k_0} | \boldsymbol{u}_{\text{synth}}^{0,1} | \cdots | \boldsymbol{u}_{\text{synth}}^{0,N_\text{synth}} | \boldsymbol{u}_{h}^{k_1} | \cdots | \boldsymbol{u}_{h}^{k_{N_c-1}}].
\end{equation}
This enriched dataset provides a denser sampling of the solution manifold, offering a more comprehensive representation of the system's evolution.

A possible use of $\mathbf{S}_{\text{synth}}$ is as the basis for POD to $\mathbf{S}_{\text{synth}}$ to obtain a reduced basis $\mathbf{U}_r \in \mathbb{R}^{N_h \times N_r}$:
\begin{equation}
    \mathbf{U}_r = \text{POD}(\mathbf{S}_{\text{synth}}, N_r).
\end{equation}
The resulting reduced basis and augmented dataset provide a rich foundation for developing various non-intrusive ROM techniques, potentially improving their accuracy and efficiency by incorporating knowledge from both the original checkpoints and the OT-based interpolated states.


==> sections/intro.tex <==
\section{Introduction}
\label{sec:intro}
The modeling and simulation of complex dynamical systems, which are often characterized by nonlinear dynamics and high-dimensional state spaces, pose significant challenges. Traditional full-order models (FOMs), such as Finite Element and Finite Volume (FV) methods, offer high accuracy but come with significant computational costs.
While high-performance computing facilities can alleviate some of these computational demands \cite{hpc-book}, computing power alone is often not sufficient for real-time simulation, large-scale parametric studies, and efficient uncertainty quantification. Since complex dynamical systems are ubiquitous in Science and Engineering, coupled with tight deadlines and the need to quantify uncertainties in the results, there is an urgent need for more efficient modeling approaches.

Reduced-order models (ROMs) have emerged as a powerful surrogate strategy to alleviate computational bottlenecks, providing rapid evaluations while maintaining accuracy \cite{Benner2015,benner2017model,Grepl2007,schilders,Rozza2008,Lassila2014,Hesthaven2016,Quarteroni2016}. ROMs have been successfully applied across various domains \cite{vol3}, including fluid dynamics \cite{aromabook}, structural mechanics \cite{Farhat2014}, and electromagnetic systems \cite{Wittig2006}. Despite their widespread success, standard ROM techniques face significant challenges when dealing with highly nonlinear, advection-dominated phenomena \cite{Greif2019}. These challenges are particularly evident in systems characterized by moving discontinuities, steep gradients, and traveling waves. Such features often result in a slow decay of the Kolmogorov n-width, which describes the error arising from a projection onto the best-possible linear subspace of a given dimension \cite{Cohen15}.

This slow decay limits the efficacy of linear ROMs and has spurred several research directions, including shifted Proper Orthogonal Decomposition (POD) \cite{Reiss2018,Papapicco2022}, calibration methodologies \cite{nonino2024calibrationbased}, and registration methods \cite{Taddei2020,Ferrero2022}. Additionally, the development of nonlinear ROMs has marked a significant advancement, particularly through the use of deep learning frameworks that efficiently extract relevant features from high-dimensional data \cite{Goodfellow2016}. Novel architectures, such as recurrent neural networks \cite{Maulik2021}, convolutional autoencoders \cite{LeeModelReductionDynamical2020,romor2023,fresca2021} and graph-based approaches \cite{PichiGraphConvolutionalAutoencoder2023,romor2023friedrichs,MorrisonGFNGraphFeedforward2024}, have further refined the potential of neural networks for regression tasks, enabling more flexible and efficient ROMs.

In this paper, we introduce a novel data-driven ROM  for highly nonlinear, advection-dominated systems by incorporating concepts from Optimal Transport (OT) theory \cite{Villani2008}, specifically leveraging displacement interpolation. The ROM is designed to handle both nonlinear dynamics and limited data scenarios, which are common challenges in many practical applications. The key elements of our methodology include an OT-based data augmentation strategy, a time-interpolation parameter mapping, and a correction step to de-bias the barycentric representation. The resulting framework generates physically consistent synthetic data used for a non-intrusive ROM approach able to capture complex nonlinear dynamics efficiently across continuous time scales.

The first step in our methodology is the selection of checkpoints from the original solution snapshots and the computation of OT plans between consecutive checkpoints. These OT plans are crucial for leveraging displacement interpolation to generate synthetic snapshots, allowing for continuous and geometrically coherent transitions between computed solutions. This process enriches the model space with synthetic solutions that are not restricted to the support of the original data snapshots. Moreover, this strategy significantly increases the amount of data available for training, enriching the POD basis, enhancing its expressivity, and improving accuracy at finer temporal scales than those of the original snapshots. Similarly, our approach could be exploited for deep learning-based approaches in model order reduction, where large datasets are crucial but only a limited amount of full-order solutions can be computed.

To construct a ROM capable of continuous inference, we need to establish mappings between the interpolation parameter and physical time. We propose both a linear mapping and an optimal regression approach, balancing flexibility and accuracy. This allows for efficient online prediction at arbitrary time points. As a correction step, we perform POD with regression (POD-R) of the residuals. A Gaussian Process Regression (GPR) model \cite{Rasmussen2004} is trained to predict the POD coefficients of these residuals, compensating for systematic biases in the OT-based interpolation.

The integration of optimal transport with ROMs builds upon recent works in this direction, including interpolation in the general L2-Wasserstein space \cite{mula2020,mula2022}, solution approximation using Wasserstein Barycenters \cite{mula2023,agueh2011barycenters}, alignment of features using OT mappings \cite{Blickhan23}, and the use of the Wasserstein kernel within kPOD reduction \cite{Khamlich23}. Notably relevant to the design of our methodology is work on convex displacement interpolation \cite{Iollo22}, which has been extended in \cite{cucchiara2023model} where nonlinear interpolation is used for data augmentation, focusing on OT maps between Gaussian models. In our approach, we consider the OT problem in its entropic regularized form, popularized through the use of the Sinkhorn algorithm \cite{cuturi13}. Specifically, we use the multiscale formulation proposed in \cite{Schmitzer2019}, which is particularly useful for problems involving vanishing entropy since it overcomes numerical instabilities, slow convergence, and excessive blurring typical of the standard implementations \cite{Peyre2019}.

While the methodology is general and applicable to a wide range of nonlinear dynamical systems, we choose to demonstrate its effectiveness for the simulation of mesoscale atmospheric flow, modeled by the weakly compressible compressible Euler equations. We focus on two classical benchmarks: the smooth rising thermal bubble and the density current. Both benchmarks are challenging as the dynamics is highly nonlinear and there is strong advection dominance, and hence are ideal to test our methodology.

The rest of the paper is organized as follows: Section \ref{sec:rom-model} introduces the general ROM framework of time-dependent problems. Section \ref{sec:ot} provides background on optimal transport and displacement interpolation. Section \ref{sec:ot_rom_framework} details our OT-based ROM framework, including the data augmentation strategy and the non-intrusive nature of the approach. Section \ref{sec:FOM} describes the FOM for the above-mentioned atmospheric benchmarks. Section \ref{sec:numerical_results} presents the numerical results obtained with our ROM and discusses the effectiveness of the methodology. Finally, Section \ref{sec:conclusions} offers conclusions and perspectives for future work.



==> sections/intro_new.tex <==
\section{Introduction}
\label{sec:intro}
The modeling and simulation of complex dynamical systems play a crucial role in modern scientific and engineering practices. These systems, often characterized by nonlinear dynamics and high-dimensional state spaces, pose significant computational challenges \cite{Benner2015,benner2017model}. Traditional full-order models (FOMs), while accurate, are frequently computationally prohibitive for real-time applications, uncertainty quantification, and large-scale parameter studies \cite{Grepl2007,schilders}.

Reduced-order models (ROMs) have emerged as a powerful approach to alleviate such computational bottlenecks, providing rapid model evaluations with minimal loss of accuracy \cite{Rozza2008,Lassila2014}. ROMs have been successfully applied across various domains, including fluid dynamics \cite{Brunton2020}, structural mechanics \cite{Farhat2015}, and electromagnetic systems \cite{Benner2014}. However, despite their widespread success, standard ROM techniques face significant challenges when dealing with highly nonlinear, advection-dominated phenomena \cite{Greif2019}.

These challenges are particularly evident in systems characterized by moving discontinuities, steep gradients, and traveling waves. Such features often result in a slow decay of the Kolmogorov n-width, which quantifies the compactness of solution manifolds within linear subspace approximations \cite{Cohen15}. This slow decay limits the efficacy of linear ROMs and has spurred several research directions, including shifted Proper Orthogonal Decomposition (POD) \cite{Reiss2018,Papapicco2022}, calibration methodologies \cite{nonino2024calibrationbased}, and registration methods \cite{Taddei2020,Ferrero2022}. Additionally, the development of nonlinear ROMs has marked a significant advancement, particularly through the use of deep learning frameworks that efficiently extract relevant features from high-dimensional data \cite{Goodfellow2016}. Novel architectures, such as recurrent neural networks \cite{Maulik2021}, convolutional autoencoders \cite{LeeModelReductionDynamical2020,romor2023,fresca2021} and graph-based approaches \cite{PichiGraphConvolutionalAutoencoder2023,romor2023friedrichs,MorrisonGFNGraphFeedforward2024}, have further refined the potential of neural networks for regression tasks, enabling more flexible and efficient ROMs.

In this paper, we introduce a novel data-driven ROM by incorporating concepts from Optimal Transport (OT) theory \cite{Villani2008}, specifically leveraging displacement interpolation. This method offers a significant advancement in handling nonlinear dynamics and limited data scenarios, which are common challenges in many scientific and engineering applications. The key elements of our methodology include an OT-based data augmentation strategy, a time-interpolation parameter mapping, and a correction step to debias the barycentric representation.

Our methodology begins by selecting checkpoints from the original solution snapshots and computing OT plans between consecutive checkpoints. These OT plans are crucial for leveraging displacement interpolation to generate synthetic snapshots, allowing for continuous and geometrically coherent transitions between probability distributions. This process enriches the model space with synthetic solutions that are not bound to the support of the original data snapshots. These synthetic solutions significantly increase the amount of data available for training, which is essential for deep learning-based ROMs where large datasets are crucial \cite{Goodfellow2016}. Moreover, they enrich the POD basis, enhancing its expressivity from a small number of physical snapshots and improving accuracy at finer temporal scales than those of the original snapshots.

To construct a ROM capable of continuous inference, we develop mappings between the interpolation parameter and physical time. We propose both a linear mapping and an optimal regression approach, offering flexibility in this time-parameter relationship. This allows for efficient online prediction at arbitrary time points. To further improve prediction accuracy and debias the barycentric representation, we introduce a correction step based on POD with regression (POD-R) of the residuals. A Gaussian Process Regression (GPR) model is trained to predict the POD coefficients of these residuals, compensating for systematic biases in the OT-based interpolation.


This comprehensive framework not only provides a method for generating physically consistent synthetic data but also enables a non-intrusive ROM approach capable of capturing complex nonlinear dynamics efficiently across continuous time scales.


The integration of optimal transport with ROMs builds upon recent works in this direction, including interpolation in the general L2-Wasserstein space \cite{mula2020,mula2022}, solution approximation using Wasserstein Barycenters \cite{mula2023,agueh2011barycenters}, alignment of features using OT mappings \cite{Blickhan23}, and the use of the Wasserstein kernel within kPOD reduction \cite{Khamlich23}. Notably relevant to this work is the research on convex displacement interpolation \cite{Iollo22}, which has been extended in \cite{cucchiara2023model}. The latter work proposes using nonlinear interpolation for data augmentation, focusing on OT maps between Gaussian models. In contrast, here we consider the OT problem in its entropic regularized form, popularized through the use of the Sinkhorn algorithm \cite{cuturi13}. Specifically, we use the multiscale formulation proposed \cite{Schmitzer2019}, which is particularly useful for problems involving vanishing entropy, since it overcome numerical instabilities, slow convergence and excessive blurring typical of the standard implementations \cite{Peyre2019}.

While the methodology is general and applicable to a wide range of nonlinear dynamical systems, we demonstrate its effectiveness using atmospheric mesoscale simulations as a challenging benchmark, showcasing its potential for handling highly nonlinear and advection-dominated phenomena.

The rest of the paper is organized as follows: Section \ref{sec:rom-model} introduces the general framework for reduced-order modeling of time-dependent problems. Section \ref{sec:ot} provides background on optimal transport and displacement interpolation. Section \ref{sec:ot_rom_framework} details our OT-based ROM framework, including the data augmentation strategy and non-intrusive modeling approach. Section \ref{sec:FOM} describes the full-order model for the atmospheric flow problems considered in this work. Section \ref{sec:numerical_results} presents numerical experiments demonstrating the method's effectiveness on atmospheric flow benchmarks. Finally, Section \ref{sec:conclusions} offers conclusions and perspectives for future work.

\anna{Metto qui sotto del materiale che sposterei nell'intro}

Although the Smagorinsky model assumes a local balance between subgrid-scale energy production and dissipation, it has notable limitations \cite{book_les}. The more refined model used in the present work is the one-equation eddy-viscosity model (kEqn model) \cite{Yoshizawa1985}, which accounts for the production, dissipation, and diffusion of subgrid-scale kinetic energy


==> sections/kpod.tex <==
\section{Kernel Proper Orthogonal Decomposition (kPOD)}
\label{sec:kpod}

The Kernel Proper Orthogonal Decomposition (kPOD) algorithm \cite{kpca} is a kernel-based extension of the classical POD algorithm.
kPOD leverages the idea that datasets with nonlinearly separable attributes can be embedded into a higher-dimensional feature space, where the information becomes more spread out and easier to compress through POD.
When projected back to the original space, the resulting modes yield a nonlinear projection that better represents the data. To avoid the explicit calculation of the higher-dimensional coordinates, kPOD uses the kernel function to implicitly map the data to the feature space, reducing the method's computational complexity. As a result, kPOD can perform the computation in the original space while still benefiting from the advantages of the nonlinear projection.

We will describe the method starting from the description of POD, which relies on the Singular Value Decomposition (SVD) of the snapshot matrix $\mathbf{S}$ defined in \eqref{eq:snap}. The SVD provides a factorization of $\mathbf{S} \in \mathbb{R}^{N_{h}\times N_{s}}$ into the form:
\begin{equation}
 \mathbf{S} = \mathbf{U} \mathbf{\Sigma} \mathbf{V^{T}},
\end{equation}
 where $\mathbf{U} \in \mathbb{R}^{N_{h}\times N_{h}}$ and $\mathbf{V} \in \mathbb{R}^{N_{s}\times N_{s}}$ are orthogonal matrices, and $\mathbf{\Sigma} \in \mathbb{R}^{N_{h}\times N_{s}}$ is a diagonal matrix.

 Let $\mathbf{U}^\star = [\boldsymbol{\varphi}_1 | \boldsymbol{\varphi}_2| \ \cdots| \ \boldsymbol{\varphi}_k] \in \mathbb{R}^{N_h \times k}$ be the truncated matrix consisting of the first $k$ columns of $\mathbf{U}$. The low-dimensional representation of a snapshot is given by $\boldsymbol{z} = \mathbf{U^{\star T}} \boldsymbol{u}_{h} \in \mathbb{R}^k$, so that the samples in $\mathbf{S}$ are mapped to $\mathbf{Z} = \mathbf{U^{\star T}} \mathbf{S} \in \mathbb{R}^{k \times N_s}$. The reduced order model is interpreted as looking for an approximation to $\boldsymbol{u}_{h}$ in the $k$-dimensional linear subspace generated by the basis $\{\boldsymbol{\varphi}_j\}_{j = 1}^{k}$. Notice that the SVD of the snapshot matrix $\mathbf{S}$ directly provides a diagonalization of the Gram matrix $\mathbf{G} = \mathbf{S^T} \mathbf{S} \in \mathbb{R}^{N_s \times N_s}$ as follows:

\begin{equation}
    \label{eig-prob-G}
    \mathbf{G} = \mathbf{V}\mathbf{[\Sigma ^T \Sigma]V ^ T = V \Lambda V ^T},
\end{equation}
where $\mathbf{\Lambda}$ is a diagonal matrix with the eigenvalues of $\mathbf{G}$ on its diagonal. In particular, the compact expression for constructing $\mathbf{Z}$  is given in terms of the Gram matrix as follows:

\begin{equation}
\label{kpod-reduction}
\mathbf{Z=V ^{\star  T} G} ,
\end{equation}
where $\mathbf{V}^\star \in \mathbb{R}^{N_s \times k}$ is the matrix consisting of the first $k$ columns of $\mathbf{V}$.

To apply kPOD, we first introduce an arbitrary transformation $\Phi: \mathbb{R}^{N_{h}} \rightarrow \mathbb{R}^{N_{H}}$ that maps the original data to a higher-dimensional feature space, where nonlinearities may become linear. Let us assume to have $N_s$ transformed snapshots $\{\Phi(\boldsymbol{u}^{j}_{h})\}_{j = 1}^{N_{s}}$, from which we can define the matrix $\tilde{\mathbf{S}} = [\Phi(\boldsymbol{u}^1_{h})| \Phi(\boldsymbol{u}^2_{h})| ... | \Phi(\boldsymbol{u}^{N_s}_{h})] \in \mathbb{R}^{N_H \times N_s}$. We aim at performing POD on $\tilde{\mathbf{S}}$ to extract a low-dimensional linear subspace that captures most of the information in the transformed snapshots.

However, computing the SVD of $\tilde{\mathbf{S}}$ directly may be computationally prohibitive if $N_{H}$ is very large, and we do not know the optimal choice of $\Phi$ that would allow us to untangle the underlying nonlinear manifold. Instead, we can compute the transformed Gram matrix $\tilde{\mathbf{G}}$ by introducing a bivariate symmetric form $\kappa(\cdot,\cdot): \mathbb{R}^{N_{h}} \times \mathbb{R}^{N_{h}} \rightarrow \mathbb{R}^k$ called \textit{kernel function} that acts as a proxy for the inner product in the high-dimensional feature space, but takes as argument the pre-image of the transformed samples:

\begin{equation}
    [\tilde{\mathbf{G}}]_{ij} = \langle \Phi(\boldsymbol{u}^{i}_{h}), \Phi(\boldsymbol{u}^{j}_{h}) \rangle = \kappa(\boldsymbol{u}^{i}_{h},\boldsymbol{u}^{j}_{h}).
\end{equation}
By doing so, we can still rely on \eqref{eig-prob-G} to obtain $\tilde{\mathbf{V}}^{\star}$ and use \eqref{kpod-reduction} to perform the model order reduction task.
In particular, we can introduce the so-called \textit{forward mapping} F:

\begin{equation}
\label{forward-map}
\begin{aligned}
F: \mathbb{R}^{N_{h}} & \rightarrow \mathbb{R}^k, \\
{\boldsymbol{u}_{h}} & \mapsto {\boldsymbol{z}} = {\tilde{\mathbf{V}}}^{\mathbf{\star T}}  {g}({\boldsymbol{u}_{h}}), \qquad {g}({\boldsymbol{u}_{h}}) = [\kappa({\boldsymbol{u}_{h}}, {\boldsymbol{u}^{i}_{h}})]_{i=1}^{N_s} \ .
\end{aligned}
\end{equation}
%\todofp{Non abbiamo definito ${\tilde{\mathbf{V}}}^{\mathbf{\star T}}$}
However, we do not have an explicit expression for the kPOD modes, which would be contained in the unknown matrix $\tilde{\mathbf{U}}$. This represents a significant problem because having only $\tilde{\mathbf{V}}^{\star}$ does not allow us to correctly map backward an element $\boldsymbol{z} \in \mathbb{R}^k$ into its pre-image $\tilde{\boldsymbol{u}}_{h} \in \mathbb{R}^{N_{h}}$.
For a more detailed description of kPOD and the various strategies for defining a backward map, we recommend interested readers to refer to \cite{kpca,Dez2021}.

A crucial aspect consists in determining the backward mapping of the low-dimensional manifold with kPOD, which is less trivial than in the standard POD framework. In particular, defining the inverse of the forward mapping $F$ requires the selection of a proper target space $\mathcal{V} \subset \mathbb{R}^{N_{h}}$ where pre-images are sought. The \textit{backward mapping} is then defined as:

\begin{equation}
    \tilde{\boldsymbol{u}}_{h}=F^{-1}(\boldsymbol{z})\stackrel{\text { def }}{=}\arg \min _{\boldsymbol{u}_{h} \in \mathcal{V}}\|F(\boldsymbol{u}_{h})-\boldsymbol{z}\|.
\end{equation}
The definition of the backward mapping depends on the selection of the manifold $\mathcal{V}$ and the approximation criterion, which is the choice of the norm $\|\cdot\|$. We remark that, since $F$ is not injective, different $\tilde{\boldsymbol{u}}_{h} \in \mathbb{R}^{N_{h}}$ can have the same image $\boldsymbol{z}$, thus, the target space must be a proper low-dimensional manifold for the backward map to be well-defined.

To address this problem, we propose to use a regression approach based on Neural Networks (NN) \cite{goodfellow,freeman1991neural}. Specifically, we will use autoencoders \cite{autoencoder}, which have been shown to be effective in solving the inverse problem originated from kPOD.


==> sections/methodology.tex <==
\subsection{Optimal Transport}

Optimal transport (OT) theory studies the problem of transporting one probability distribution onto another with minimum cost. The cost is usually measured by a distance function $d$, which quantifies the dissimilarity between the two distributions. The Wasserstein distance, also known as the earth mover's distance, is a popular choice of distance function in OT, as it provides a way to compare probability distributions in a metric space. Given two probability measures $\mu$ and $\nu$ on a metric space $\mathcal{X}$, their $p$-th order Wasserstein distance $W_p(\mu, \nu)$ is defined as

\begin{equation}
W_p(\mu, \nu) = \left(\inf_{\gamma \in \Gamma(\mu, \nu)} \int_{\mathcal{X} \times \mathcal{X}} d(x,y)^p d\gamma(x,y) \right)^{1/p},
\end{equation}

where $\Gamma(\mu, \nu)$ is the set of all joint probability measures on $\mathcal{X} \times \mathcal{X}$ with marginals $\mu$ and $\nu$. Intuitively, $W_p(\mu, \nu)$ measures the minimum amount of "work" needed to transform $\mu$ into $\nu$, where the amount of work is weighted by the cost function $d$ raised to the power $p$.

A transport map $T:\mathcal{X} \rightarrow \mathcal{Y}$ is a function that maps each point $x \in \mathcal{X}$ to a point $y \in \mathcal{Y}$, such that $\mu$ is transported to $\nu$ via $T$. The optimal transport map $T^*$ can be obtained using the Kantorovich-Rubinstein duality, which relates the Wasserstein distance to a linear programming problem.

The duality theorem states that the $p$-Wasserstein distance between $\mu$ and $\nu$ can be expressed as the supremum of the dual problem over a certain set of functions, known as the Kantorovich potentials. The dual problem is a linear programming problem that involves finding the infimum of a certain functional over a set of measures. The set of measures corresponds to the set of joint probability measures with marginals $\mu$ and $\nu$, denoted by $\Gamma(\mu,\nu)$. The functional is defined in terms of the Kantorovich potentials, which are functions that map points in $\mathcal{X}$ to real numbers.

More specifically, the dual problem can be formulated as

\begin{equation}
\label{eq:dual_problem}
\inf_{\gamma \in \Gamma(\mu, \nu)} \int_{\mathcal{X} \times \mathcal{X}} c(x,y) d\gamma(x,y),
\end{equation}

where $c(x,y)$ is a cost function that measures the cost of transporting a unit of mass from $x$ to $y$.

\subsection{Entropic Regularization and Sinkhorn Algorithm}

The computation of the Wasserstein distance is a nontrivial task, especially for high-dimensional data. However, the Sinkhorn algorithm provides an efficient and scalable method for computing the Wasserstein distance. The Sinkhorn algorithm is based on entropic regularization, which introduces a small amount of entropy into the optimization problem. This regularization leads to a differentiable and convex optimization problem that can be efficiently solved using iterative methods.

The entropic regularization of the Wasserstein distance involves the introduction of a parameter $\epsilon > 0$ that controls the amount of regularization. The regularized Wasserstein distance is given by:

\begin{equation}
W_{\epsilon}(\mu, \nu) = \inf_{\gamma \in \Gamma(\mu, \nu)} \langle C, \gamma \rangle - \epsilon H(\gamma),
\label{eq:wasserstein_regularized}
\end{equation}

where $\Gamma(\mu, \nu)$ is the set of probability measures on $\mathcal{X} \times \mathcal{Y}$ with marginals $\mu$ and $\nu$, $C$ is the cost function, and $H(\gamma)$ is the entropy of the transport plan $\gamma$:

\begin{equation}
H(\gamma) = -\int_{\mathcal{X} \times \mathcal{Y}} \log(\gamma(x,y)) , \mathrm{d}\gamma(x,y).
\label{eq:entropy}
\end{equation}

The entropic regularization introduces a smoothness term that allows for more efficient optimization. However, the optimization problem in Equation~\ref{eq:wasserstein_regularized} is still difficult to solve directly. The Sinkhorn algorithm provides an efficient method for solving this optimization problem.

The Sinkhorn algorithm is an iterative algorithm that computes a sequence of transport plans that converge to the optimal transport plan. The algorithm works by alternately scaling the rows and columns of the transport plan until convergence. The resulting sequence of transport plans is guaranteed to converge to the optimal transport plan, and the convergence rate is exponential in the number of iterations.

The Sinkhorn algorithm can be written as:

\begin{align}
u_{i}^{k+1} &= \frac{\alpha_{i}}{\langle v^{k}, K_{i} \rangle}, \label{eq:sinkhorn_scaling_u} \
v_{j}^{k+1} &= \frac{\beta_{j}}{\langle u^{k+1}, K_{j} \rangle}, \label{eq:sinkhorn_scaling_v}
\end{align}

where $K = \exp(-C/\epsilon)$ is the kernel matrix, $\alpha$ and $\beta$ are the marginal weights, and $u$ and $v$ are the scaling factors for the rows and columns, respectively. The iteration is initialized with $u_{i}^{0} = \frac{1}{m}$ and $v_{j}^{0} = \frac{1}{n}$, where $m$ and $n$ are the number of rows and columns in the kernel matrix, respectively.

The regularized Wasserstein distance can then be computed as:

\begin{equation}
W_{\epsilon}(\mu, \nu) = \langle u^{}, K \circ C \circ v^{} \rangle - \epsilon H(u^{} \otimes v^{}),
\label{eq:wasserstein_sinkhorn}
\end{equation}

where $u^{}$ and $v^{}$ are the optimal scaling factors obtained by iterating Equations
until convergence is achieved, typically measured by the duality gap or a stopping criterion.


==> sections/numerical_results.tex <==
\section{Numerical Results}
\label{sec:numerical_results}

To validate our framework, we consider two standard benchmarks for atmospheric flows in two dimensions: the rising thermal bubble with the setting from \cite{Ahmad2006} and the density current with the setting from \cite{Straka1993}.
Both test cases model a perturbation of a neutrally stratified atmosphere with uniform background potential temperature. Sec.~\ref{subsec:thermal-bubble} presents the results for the rising thermal bubble benchmark, in which the perturbation consists of warm air that rises and deforms into a mushroom shape.
Sec.~\ref{subsec:density-current} shows the results for the density current benchmark, in which the perturbation is made of cold air that falls to the ground and forms a propagating cold front.

To quantify the accuracy of our approach, we use the relative $\mathcal{L}^2$ norm in spatial domain $\Omega$, defined as:
\begin{equation}
\label{eq:l2_error}
E_{\mathcal{L}^2(\Omega)}(u_{\text{ref}}, \hat{u}) = \frac{\|u_{\text{ref}} - \hat{u}\|_{\mathcal{L}^2(\Omega)}}{\|u_{\text{ref}}\|_{\mathcal{L}^2(\Omega)}},
\end{equation}
where $u_{\text{ref}}$ is the reference solution field and $\hat{u}$ is an approximation. For both tests, the quantity of interest is the perturbation of potential temperature $\theta'$. The reference solution $\theta'_{\text{ref}}(t)$ is obtained with a fine time step $\Delta t_{\text{ref}}$.

To generate the approximation, we introduce a second coarser time step $\Delta t_{\text{train}} = m \Delta t_{\text{ref}}$, for some integer $m > 1$, and denote with $\theta'_{\text{train}}(t)$ the training solution.
We define the set of training time points as $\mathcal{T}_{\text{train}} = \{t_k = k\Delta t_{\text{save}} \mid k = 1, ..., N_T\}$, where $\Delta t_{\text{save}} = n \Delta t_{\text{train}}$ for some integer $n \geq 1$.
The corresponding training dataset is given by $\mathcal{S}_{\text{train}} = \{\theta'_{\text{train}}(t_k) \mid t_k \in \mathcal{T}_{\text{train}}\}$.
To evaluate our method's capability across different time discretizations, we define a set of test points $\mathcal{T}_{\text{test}}$ that has no intersection with $\mathcal{T}_{\text{train}}$ and
denoted with $\mathcal{S}_{\text{test}} = \{\theta'_{\text{ref}}(t_j) \mid t_j \in \mathcal{T}_{\text{test}}\}$
the corresponding test dataset.

The following error metrics will be considered.
The coarser discretization introduces an intrinsic error quantified by the time \emph{discretization error}:
\begin{align}
E_{\text{disc}}(t_k, \Delta t_{\text{train}}) &= E_{\mathcal{L}^2(\Omega)}(\theta'_{\text{train}}(t_k),\theta'_{\text{ref}}(t_k)), \quad t_k \in \mathcal{T}_{\text{train}}, \cl
\overline{E}_{\text{disc}}(\Delta t_{\text{train}}) &= \frac{1}{|\mathcal{T}_{\text{train}}|} \sum_{t_k \in \mathcal{T}_{\text{train}}} E_{\text{disc}}(t_k, \Delta t_{\text{train}}), \el
\end{align}
where $E_{\text{disc}}$ is the pointwise error and $\overline{E}_{\text{disc}}$ is its mean across time.

The \textit{interpolation error} quantifies the accuracy of our synthetic snapshots interpolating the training data:
\begin{equation}
E_{\text{interp}}(\mathcal{F}, t_k) = E_{\mathcal{L}^2(\Omega)}(\boldsymbol{u}_{\text{synth}}(\mathcal{F}_1(t_k), \mathcal{F}_2(t_k)), \theta'_{\text{train}}(t_k)), \quad t_k \in \mathcal{T}_{\text{train}} ,
\end{equation}
where $\mathcal{F} \in \{\mathcal{M}, \mathcal{L}\}$ represents either the MinL2 regression mapping $\mathcal{M}$ or the linear mapping $\mathcal{L}$, as explained in Sec.~\ref{sec:ot_rom_framework}, and
% $\mathcal{F}_1$ and $\mathcal{F}_2$ are the first and second components of the respective mapping.
$\boldsymbol{u}_{\text{synth}}$ is the synthetic snapshot generation function defined in eq.~\eqref{eq:online_inference}.
The \textit{generalization error} measures how well our synthetic snapshots approximate the reference solution:
\begin{equation}
E_{\text{gen}}(\mathcal{F}, t_j) = E_{\mathcal{L}^2(\Omega)}(\boldsymbol{u}_{\text{synth}}(\mathcal{F}_1(t_j), \mathcal{F}_2(t_j)), \theta'_{\text{ref}}(t_j)), \quad t_j \in \mathcal{T}_{\text{test}}.
\end{equation}
It is important to note that the generalization error represents a cross-discretization comparison, evaluating our method's ability to approximate the finer reference solution using coarser training data for time instances unseen during training.
For both error types, we report the mean error:
\begin{equation}
\overline{E}_{\text{type}}(\mathcal{F}) = \frac{1}{|\mathcal{T}|} \sum_{t \in \mathcal{T}} E_{\text{type}}(\mathcal{F}, t), \quad \text{type} \in \{\text{interp}, \text{gen}\},
\end{equation}
where $\mathcal{T}$ is the corresponding set of time points for each error type.

\vskip .2cm
\noindent {\bf Computational Setup}.
For the numerical solution of the rising thermal bubble and density current benchmarks, we  used
GEA\footnote{The source code of GEA can be found in \url{https://github.com/GEA-Geophysical-and-Environmental-Apps/GEA}} - Geophysical and Environmental Applications \cite{GEA,girfoglio2024comparative, Girfoglio_2023}, an open-source software package for atmospheric and oceanic modeling based on
the OpenFOAM library \cite{openfoam}.
For the OT problems, we used the MultiScaleOT library \cite{multiscale-ot} which implements stabilized sparse scaling algorithms for entropy regularized transport problems \cite{Schmitzer2019}.
The experiments were performed on a machine equipped with an NVIDIA GeForce RTX 3080 GPU and an 11th Gen Intel(R) Core(TM) i7-11700 @ 2.50GHz processor running Rocky Linux version 8.8.

\input{sections/thermal-bubble}
\input{sections/density-current}


==> sections/old_intro.tex <==
\section{Old Introduction}
\label{sec:old_intro}


In recent years, we have experienced a sustained increase in computational capabilities; however, atmospheric flow simulations through traditional discretization methods, such as finite element methods or finite volume methods, remain computationally expensive. The need to perform a large number of simulations for quantifying uncertainty in weather forecasts requires alternatives to such discretization methodologies, also known as full-order models (FOMs), to reduce computational time and improve forecast reliability in short time.

Reduced-order models (ROMs) have emerged as a preferred methodology to relieve computational load when FOM simulations need to be run for different values of physical parameters, as in uncertainty quantification, or for long periods of time, as in weather forecasting. ROMs replace the chosen FOM with a lower-dimensional approximation that captures the essential behavior of the system. This is accomplished through a two-stage procedure: in the first stage, called the offline stage, a database of different FOM solutions associated with specific times and/or physical parameter values is constructed. The database of FOM solutions is used to generate a reduced base, with very small cardinality compared to the high dimensionality of the FOM but still preserving the essential features of the evolution of the system with respect to the physical and geometric parameters that encode it. In the second phase, called the online phase, this reduced basis is used to rapidly compute the solution for new times and/or values of the specified parameters.

ROMs successfully applied to fluid dynamics problems can be divided into two main categories: projection-based and data-driven. The former project the governing equations onto a low-dimensionality space defined by the reduced basis functions. The latter, on the other hand, rely on the available high-dimensionality FOM system data to directly learn a reduced-order model without explicitly considering the underlying equations.

In this paper, we focus on data-driven ROMs. The efficiency of projection-based ROMs is rather limited in the case of nonlinear problems, which often require hyper-reduction techniques that are problem-dependent and computationally expensive. Therefore, nonintrusive ROMs are preferred for applications where a high degree of acceleration is required.

Since atmospheric flows are strongly nonlinear and high speed-up is desirable for prediction, the objective of this paper is to further improve data-driven ROMs by introducing a new approach based on interpolation by displacement, a concept derived from the field of optimal transport. This interpolation technique has a key feature: it allows continuous interpolation between probability distributions, generating interpolated solutions that do not reside on the support of reference snapshots, but whose support follows a geodesic in the space of probability distributions connecting the extremes. This approach makes it possible to generate synthetic solutions that increase the amount of data available for training, which is essential in contexts such as deep learning-based ROMs (DL-ROMs), where the availability of large datasets is crucial. Such synthetic solutions can not only enrich a POD basis, making it more expressive from a small number of physical snapshots, but can also more accurately approximate physical solutions using finer temporal discretization than the original snapshots used for interpolation. This is particularly relevant for dealing with PDEs that present significant challenges due to predominant convection phenomena, as demonstrated by the two dry atmosphere benchmarks considered in this study.


==> sections/optimal_transport.tex <==
\section{Optimal Transport Theory}
\label{sec:ot}

Optimal Transport (OT) theory is a mathematical framework dedicated to solving transport problems, finding applications in fields such as probability, economics, image recognition, and machine learning. The Monge formulation of OT seeks to identify an optimal mapping that minimizes transportation costs between two probability distributions, represented as $\mu$ and $\nu$. These distributions occupy metric spaces $\mathcal{X}$ and $\mathcal{Y}$, with the transportation cost from $\mathcal{X}$ to $\mathcal{Y}$ quantified by a cost function $c: \mathcal{X} \times \mathcal{Y} \rightarrow \mathbb{R}^+$.

For a measurable function $T: \mathcal{X} \rightarrow \mathcal{Y}$ that defines the push-forward measure $T_\mu$ on $\mathcal{Y}$, where $T_\mu(A) = \mu(T^{-1}(A))$ for any measurable set $A \subset \mathcal{Y}$, $T$ is termed a \textit{transport map} if it satisfies $T_\mu = \nu$. The objective is to find the transport map $T^*$ that minimizes the total cost:


\begin{equation}
    T^* = \argmin_{T \ \text{s.t.}\ T_\#\mu = \nu} \int_{\mathcal{X}} c(x ; T(x)) d \mu .
\end{equation}


The Kantorovich formulation introduces a generalization by focusing on \textit{transport plans} rather than direct mappings. A transport plan $\pi$ is a measure on $\mathcal{X} \times \mathcal{Y}$ that dictates the transfer of mass in alignment with the marginal distributions $\mu$ and $\nu$.

The optimization challenge, according to Kantorovich, is to find the optimal transport plan $\pi^*$ that minimizes:

\begin{equation}
    \pi ^* = \argmin_{\pi \in \Pi(\mu,\nu)}\int_{\mathcal{X}\times \mathcal{Y}}c(x, y)d\pi(x,y).
\end{equation}


This approach is advantageous for its ability to handle partial transportation scenarios, making it highly adaptable for real-world applications.

The \textit{Wasserstein distance} then becomes a key metric in OT, quantifying the minimal transport cost between distributions. In the discrete case, the problem simplifies to linear programming, solvable through various optimization techniques.

\subsection{Entropic Regularization and Sinkhorn Algorithm}
\label{subsec:sink}

Computing the Wasserstein distance is a nontrivial task, especially for high-dimensional data. However, the Sinkhorn algorithm, exploiting entropic regularization, provides an efficient and scalable method for its computation.

The entropic regularization introduces a small amount of entropy into the optimization problem, leading to a differentiable and convex optimization problem that can be efficiently solved using iterative methods.
This procedure introduces a parameter $\epsilon > 0$ that controls the amount of regularization (see Figure \ref{fig:sink_}).

The regularized Wasserstein distance is given by:
\begin{equation}
    W_{\text{reg}}(\mu, \nu) \stackrel{\text { def }}{=} \min_{\boldsymbol{\pi} \in \Pi_{\text{dis}}(\mu, \nu)} \langle \mathbf{C}, \boldsymbol{\pi} \rangle - \epsilon H(\boldsymbol{\pi}),
\label{eq:wasserstein_regularized}
\end{equation}
where $H(\pi)$ is the \textit{Shannon entropy} of the transport plan $\pi$, defined as:
\begin{equation}
    H(\boldsymbol{\pi}) \stackrel{\text { def }}{=} - \sum_{i = 1} ^n \sum _{j = 1}^m \boldsymbol{\pi}_{ij}
 (\log(\boldsymbol{\pi}_{ij})-1).
 \label{eq:entropy}
\end{equation}
The entropic regularization introduces the smoothing term
$H(\boldsymbol{\pi})$, which is uniformly concave with respect to its argument.


This allows for more efficient optimization since the regularized Problem
\eqref{eq:wasserstein_regularized} is uniformly convex and thus admits a unique
minimum.
%
To achieve the optimum for \eqref{eq:wasserstein_regularized}, a first simplification lies in writing the corresponding Karush-Kuhn-Tucker \cite{Rockafellar1970}
conditions. Doing so yields
the following characterization:
\begin{equation}
 \boldsymbol{\pi}^* \text { solution to \eqref{eq:wasserstein_regularized} } \Leftrightarrow\left\{\begin{array}{l}
        \boldsymbol{\pi}^* \in \Pi_{\text{dis}}(\mu,\nu) , \\
  \mathbf{K} \in \mathbb{R}_+^{n \times m}: \quad \mathbf{K}_{ij} = e^{\frac{\mathbf{C}_{ij}}{\epsilon}},\\
        \exists\ \boldsymbol{u} \in \mathbb{R}^n,\ \boldsymbol{v} \in \mathbb{R}^m: \quad \boldsymbol{\pi}^{*}_{ij}=\boldsymbol{u}_i \mathbf{K}_{ij} \boldsymbol{v}_j.
\end{array} \right.
\label{ktt-conditions}
\end{equation}
Thanks to the equivalence provided by \eqref{ktt-conditions}, one can
solve the Kantorovich problems using the Sinkhorn-Knopp's fixed point iteration
\cite{sink} reported in Algorithm \ref{alg-sink}.  The algorithm works by
iteratively scaling the rows and columns of the transport plan until
convergence. The resulting sequence of transport plans is guaranteed to
converge to the optimal one.

\begin{algorithm2e}[h]
\SetAlgoLined
  \SetKwInput{Input}{Input}
  \SetKwInput{Output}{Output}
  \Input{Two probability vectors $\boldsymbol{a} \in \mathbb{R}^n$, $\boldsymbol{b} \in \mathbb{R}^m$, a cost matrix $C \in \mathbb{R}^{n \times m}$, and a regularization parameter $\epsilon > 0$}
  \Output{Optimal transport plan $\mathbf{P}$ of size $n \times m$}
  Initialize $\boldsymbol{u}^{(0)} \leftarrow \boldsymbol{1}_n$ and $\boldsymbol{v}^{(0)} \leftarrow \boldsymbol{1}_m$\ and  set $\ell \leftarrow 0$\;
  \tcp{Compute the matrix $\mathbf{K}$}
  $(\mathbf{K})_{ij} \leftarrow e^{-\frac{(\mathbf{C})_{ij}}{\epsilon}}$ for all $i$ and $j$\;
  \While{not converged}{
    \tcp{Update dual variables $u$ and $v$}
    $\boldsymbol{u}^{(\ell+1)} \leftarrow \frac{\boldsymbol{a}}{\mathbf{K} \boldsymbol{v}^{(\ell)}}$ \ and \ $\boldsymbol{v}^{(\ell+1)} \leftarrow \frac{\boldsymbol{b}}{\mathbf{K}^{\top} \boldsymbol{u}^{(\ell+1)}}$\;
    $\ell \leftarrow \ell + 1$\;
  }
  \tcp{Compute the regularized transport plan $P$ }
  $(\mathbf{P})_{ij} \leftarrow (\boldsymbol{a}^{(\ell)})_i (\mathbf{K})_{ij} (\boldsymbol{b}^{(\ell)})_j$ for all $i$ and $j$\;
\caption{Sinkhorn-Knopp's Iteration for Optimal Transport}
\label{alg-sink}
\end{algorithm2e}

Algorithm \ref{alg-sink} is iterated until convergence is achieved, as
measured by the duality gap or another stopping criterion
\cite{peyre2019computational}. The output is the regularized transport plan
$\boldsymbol{\pi}_\epsilon$ which can be used to compute the \textit{Sinkhorn
distance} \cite{cuturi13}:
\begin{equation}
W_{\epsilon}(\mu, \nu)\stackrel{\text { def }}{=}\ \langle \boldsymbol{\pi}_\epsilon,  \mathbf{C}  \rangle.
\label{eq:sinkhorn-distance}
\end{equation}
The issue with the former quantity is that, unlike the Wasserstein distance, it
can be proven to not be positive and definite. In particular, for any given target
measure $\nu$, there exist a measure $\mu$ s.t. $W_{\epsilon}(\mu, \nu)< W_{\epsilon}(\nu, \nu)\neq 0 .$

However, we can introduce additional corrective terms to debias $W_{\epsilon}$, obtaining the so-called \textit{Sinkhorn divergence} \cite{Ramdas2017,genevay2018}:
\begin{equation}
    S_{\epsilon}(\mu, \nu)\stackrel{\text { def }}{=}\ W_{\epsilon}(\nu, \mu) - \frac{1}{2}W_{\epsilon}(\nu, \mu) - \frac{1}{2}W_{\epsilon}(\nu, \mu).
\end{equation}
The previous quantity trivially satisfies $S_{\epsilon}(\mu,\mu ) = 0$, and provides a valid dissimilarity measure between two probability distributions \cite{feydy2019interpolating}.
%
Furthermore, since the computation of $S_{\epsilon}(\mu, \nu)$  only involves matrix-vector multiplications, it is highly parallelizable and can take advantage of GPUs, resulting in a significant reduction in computational cost. Algorithm \ref{alg-sink} can be further optimized to achieve a computational complexity of $\mathcal{O}(n \log n + m \log m)$ with a linear memory footprint \cite{feydy-thesis}, making it suitable for solving large-scale optimization problems.

\subsection{Multiscale Optimal transport}
\label{subsec:multiscaleot}


==> sections/pod-r.tex <==
\subsection{POD with regression}%
\label{sub:pod_with_inteporlation_podi_}

% The technique of Proper Orthogonal Decomposition with Regression (POD-R) represents a significant advancement within the ROM community for creating data-driven ROMs.
The Proper Orthogonal Decomposition with Regression (POD-R) is a data-driven reduction strategy that %circumvents the need for the physics by performing
performs a regression-task to approximate the trajectory of the full-order model. This modification not only broadens its utility to encompass scenarios where the FOM solver is not open-source, but also extends its applicability to datasets derived from experimental techniques, such as those obtained from Particle Image Velocimetry (PIV) images \cite{SemeraroAnalysisTimeresolvedPIV2012}.

The POD algorithm is used to build a reduced space $V_r$, where $\operatorname{dim}(V_r) = N_r \ll N_h$, spanned by the POD modes, i.e., the columns of the matrix $\mathbf{V} \in \mathbb{R}^{N_h \times N_r}$ such that:
\begin{equation}
\mathbf{V}=\underset{\hat{\mathbf{V}}\in \mathbb{R}^{N_r}}{\operatorname{argmin}} \frac{1}{\sqrt{N_{s}}}\left\|\mathbf{S}-\hat{\mathbf{V}} \hat{\mathbf{V}}^{\top} \mathbf{S}\right\|_{F},
\end{equation}
where $ \|\cdot\|_{F}$ denotes the Frobenius matrix norm and $\mathbf{S}$ is the snapshot matrix in \eqref{eq:snapshots_matrix}.
Thus, we can approximate the solution $\boldsymbol{u}_h(t)$, by a reduced expansion w.r.t.\ to the POD basis as:
\begin{equation}
    \label{exp-rom}
    \boldsymbol{u}_h(t)\approx \mathbf{V} \boldsymbol{\alpha}_r(t),
\end{equation}
where $\boldsymbol{\alpha}_r \in \mathbb{R}^{N_r}$ is the time-dependent vector collecting the expansion coefficients.

The POD-R method exploits a  regression approach based on the linear expansion defined in \eqref{exp-rom}. Starting from the training database $\mathcal{D} = \{(t_{j}, \boldsymbol{u}_h(t_{j}))\}_{j=1}^{N_\text{train}}$, which consists of $N_\text{train}$ pairs of time and their corresponding solution (i.e., the same to build the POD basis \anna{Non capisco, se e' lo stesso di POD perche' usiamo $N_\text{train}$ invece di $N_r$?}), each trajectory is projected onto the reduced basis to obtain the ROM coefficients:
\begin{equation}
    \boldsymbol{\alpha}_{r}(t_j) = \mathbf{V}^{\top} \boldsymbol{u}_{h}(t_j), \qquad \forall\ j=1,\dots,N_\text{train}.
\end{equation}
This gives us a database of reduced coefficients, $\mathcal{D}_{r} = \{(t_{j}, \boldsymbol{\alpha}_{r}(t_{j}))\}_{j=1}^{N_\text{train}}$, which can be used to learn a regression map $\pi: \mathcal{I} \mapsto \mathbb{R}^{N_{r}}$, approximating the function $\mathscr{F}: t \in \mathcal{I} \rightarrow \boldsymbol{\alpha}_{r}(t) \in \mathbb{R}^{N_{r}}$.

Finally, the full-order solution is reconstructed via the ``inverse'' coordinate transformation:
\begin{equation}
    \label{reconstruction}
    \boldsymbol{u}_h(t) = \mathbf{V} \pi(t).
\end{equation}

This method has been used in combination with different regression approaches, including
% considerable traction in the ROM community, finding diverse applications that vary based on the regression model used. Popular methods include
Radial Basis Function (RBF) regression \cite{xiao2015}, Gaussian Process Regression (GPR) and Artificial Neural Networks (ANNs) \cite{ubbiali}. In this study, we exploit the Gaussian Process Regression (GPR), detailed further in \cite{GuoReducedOrderModeling2018,OrtaliGaussianProcessRegression2022}.

\subsection{Proper Orthogonal Decomposition (POD)}
\label{sub:pod}

The POD algorithm is used to build a reduced space $U_r$, where $\operatorname{dim}(U_r) = N_r \ll N_h$, spanned by the POD modes, i.e., the columns of the matrix $\mathbf{U_r} \in \mathbb{R}^{N_h \times N_r}$ such that:
\begin{equation}
\mathbf{V}=\underset{\hat{\mathbf{V}}\in \mathbb{R}^{N_r}}{\operatorname{argmin}} \frac{1}{\sqrt{N_{s}}}\left\|\mathbf{S}-\hat{\mathbf{V}} \hat{\mathbf{V}}^{\top} \mathbf{S}\right\|_{F},
\end{equation}
where $ \|\cdot\|_{F}$ denotes the Frobenius matrix norm and $\mathbf{S}$ is the snapshot matrix in \eqref{eq:snapshots_matrix}.

The POD modes can be computed efficiently through the singular value decomposition (SVD) of the snapshot matrix:

\begin{equation}
\mathbf{S} = \mathbf{U}\mathbf{\Sigma}\mathbf{V}^T,
\end{equation}

where $\mathbf{U} \in \mathbb{R}^{N_h \times N_h}$ and $\mathbf{V} \in \mathbb{R}^{N_T \times N_T}$ are orthogonal matrices, and $\mathbf{\Sigma} \in \mathbb{R}^{N_h \times N_T}$ is a diagonal matrix containing the singular values $\sigma_1 \geq \sigma_2 \geq \cdots \geq \sigma_r > 0$ in descending order.

The POD modes are the left singular vectors (columns of $\mathbf{U}$) corresponding to the largest singular values. The energy captured by the first $k$ modes is given by:

\begin{equation}
E(k) = \frac{\sum_{i=1}^k \sigma_i^2}{\sum_{i=1}^r \sigma_i^2},
\end{equation}

where $r$ is the rank of $\mathbf{S}$. Typically, a reduced basis $\mathbf{U_r} \in \mathbb{R}^{N_h \times N_r}$ is constructed by selecting the first $N_r$ columns of $\mathbf{U}$, where $N_r$ is chosen such that $E(N_r)$ exceeds a desired threshold (e.g., 99.9\% of the total energy).


\subsection*{POD with Regression (POD-R)}
\label{sub:pod_r}

The Proper Orthogonal Decomposition with Regression (POD-R) is a data-driven reduction strategy that performs a regression task to approximate the trajectory of the full-order model. This modification not only broadens its utility to encompass scenarios where the FOM solver is not open-source, but also extends its applicability to datasets derived from experimental techniques, such as those obtained from Particle Image Velocimetry (PIV) images \cite{SemeraroAnalysisTimeresolvedPIV2012}.

Using the POD basis $\mathbf{U_r}$, we can approximate the solution $\boldsymbol{u}_h(t)$ by a reduced expansion:

\begin{equation}
	\label{exp-rom}
	\boldsymbol{u}_h(t)\approx \mathbf{U_r} \boldsymbol{\alpha}_r(t),
\end{equation}

where $\boldsymbol{\alpha}_r \in \mathbb{R}^{N_r}$ is the time-dependent vector collecting the expansion coefficients.

The POD-R method exploits a regression approach based on this linear expansion. Starting from the training database $\mathcal{D} = \{(t_{j}, \boldsymbol{u}_h(t_{j}))\}_{j=1}^{N_\text{train}}$, which consists of $N_\text{train}$ pairs of time and their corresponding solution, each trajectory is projected onto the reduced basis to obtain the ROM coefficients:

\begin{equation}
	\boldsymbol{\alpha}_{r}(t_j) = \mathbf{U_r}^{\top} \boldsymbol{u}_{h}(t_j), \qquad \forall\ j=1,\dots,N_\text{train}.
\end{equation}

This gives us a database of reduced coefficients, $\mathcal{D}_{r} = \{(t_{j}, \boldsymbol{\alpha}_{r}(t_{j}))\}_{j=1}^{N_\text{train}}$, which can be used to learn a regression map $\pi: \mathcal{I} \mapsto \mathbb{R}^{N_{r}}$, approximating the function $\mathscr{F}: t \in \mathcal{I} \rightarrow \boldsymbol{\alpha}_{r}(t) \in \mathbb{R}^{N_{r}}$.

Finally, the full-order solution is reconstructed via the ``inverse'' coordinate transformation:

\begin{equation}
	\label{reconstruction}
	\boldsymbol{u}_h(t) = \mathbf{U_r} \pi(t).
\end{equation}

This method has been used in combination with different regression approaches, including Radial Basis Function (RBF) regression \cite{xiao2015}, Gaussian Process Regression (GPR) and Artificial Neural Networks (ANNs) \cite{ubbiali}. In this study, we exploit the Gaussian Process Regression (GPR), detailed further in \cite{GuoReducedOrderModeling2018,OrtaliGaussianProcessRegression2022}.




==> sections/pod.tex <==
\subsection{Proper Orthogonal Decomposition (POD)}
\label{sub:pod}

The POD algorithm is used to build a reduced space $U_r$, where $\operatorname{dim}(U_r) = N_r \ll N_h$, spanned by the POD modes, i.e., the columns of the matrix $\mathbf{U_r} \in \mathbb{R}^{N_h \times N_r}$ such that:
\begin{equation}
\mathbf{U_r}=\underset{\hat{\mathbf{U}}\in \mathbb{R}^{N_h \times N_r}}{\operatorname{argmin}} \frac{1}{\sqrt{N_{T}}}\left\|\mathbf{S}-\hat{\mathbf{U}} \hat{\mathbf{U}}^{\top} \mathbf{S}\right\|_{F},
\end{equation}
where $ \|\cdot\|_{F}$ denotes the Frobenius matrix norm and $\mathbf{S}$ is the snapshot matrix in \eqref{eq:snapshots_matrix}.

The POD modes can be computed efficiently through the singular value decomposition (SVD) of the snapshot matrix:
\begin{equation}
\mathbf{S} = \mathbf{U}\mathbf{\Sigma}\mathbf{V}^T,
\end{equation}
where $\mathbf{U} \in \mathbb{R}^{N_h \times N_h}$ and $\mathbf{V} \in \mathbb{R}^{N_T \times N_T}$ are orthogonal matrices, and $\mathbf{\Sigma} \in \mathbb{R}^{N_h \times N_T}$ is a diagonal matrix containing the singular values $\sigma_1 \geq \sigma_2 \geq \cdots \geq \sigma_r > 0$ in descending order. Here, $r$ is the rank of $\mathbf{S}$.

The POD modes are the left singular vectors (i.e., the columns of $\mathbf{U}$) corresponding to the largest singular values. The  eigenvalue energy captured by the first $k$ modes is given by:
\begin{equation}
E(k) = \frac{\sum_{i=1}^k \sigma_i^2}{\sum_{i=1}^r \sigma_i^2}.
\end{equation}
Typically, a reduced basis $\mathbf{U_r} \in \mathbb{R}^{N_h \times N_r}$ is constructed by selecting the first $N_r$ columns of $\mathbf{U}$, where $N_r$ is chosen such that $E(N_r)$ exceeds a desired threshold (e.g., 99.9\% of the total eigenvalue energy).


\subsection{POD with Regression (POD-R)}
\label{sub:pod_r}

The Proper Orthogonal Decomposition with Regression (POD-R) is a data-driven reduction strategy that performs a regression task to approximate the trajectory of the full-order model. This modification not only broadens its utility to encompass scenarios where the FOM solver is not open-source, but also extends its applicability to datasets derived from experimental techniques, such as those obtained from Particle Image Velocimetry (PIV) images \cite{SemeraroAnalysisTimeresolvedPIV2012}.

Using the POD basis $\mathbf{U_r}$, we can approximate the solution $\boldsymbol{u}_h(t)$ by a reduced expansion:

\begin{equation}
	\label{exp-rom}
	\boldsymbol{u}_h(t)\approx \boldsymbol{u}_r(t) =\mathbf{U_r} \boldsymbol{\alpha}_r(t),
\end{equation}
where $\boldsymbol{\alpha}_r \in \mathbb{R}^{N_r}$ is the time-dependent vector collecting the expansion coefficients.
The POD-R method exploits a regression approach based on this linear expansion. Starting from a training database $\mathcal{D} = \{(t_{j}, \boldsymbol{u}_h(t_{j}))\}_{j=1}^{N_\text{train}}$, which consists of $N_\text{train}$ pairs of time points and their corresponding solution, each trajectory is projected onto the reduced basis to obtain the ROM coefficients:

\begin{equation}
	\boldsymbol{\alpha}_{r}(t_j) = \mathbf{U_r}^{\top} \boldsymbol{u}_{h}(t_j), \qquad \forall\ j=1,\dots,N_\text{train}.
\end{equation}
This gives us a database of reduced coefficients, $\mathcal{D}_{r} = \{(t_{j}, \boldsymbol{\alpha}_{r}(t_{j}))\}_{j=1}^{N_\text{train}}$, which can be used to learn a regression map $\pi: \mathcal{I} \mapsto \mathbb{R}^{N_{r}}$, approximating the mapping $\mathscr{F}: t \in \mathcal{I} \rightarrow \boldsymbol{\alpha}_{r}(t) \in \mathbb{R}^{N_{r}}$.

Finally, the full-order solution is reconstructed via the ``inverse'' coordinate transformation:

\begin{equation}
	\label{reconstruction}
	\boldsymbol{u}_h(t) = \mathbf{U_r} \pi(t).
\end{equation}

This method has been used in combination with different regression approaches, including Radial Basis Function (RBF) regression \cite{xiao2015}, Gaussian Process Regression (GPR) and Artificial Neural Networks (ANNs) \cite{ubbiali,PichiArtificialNeuralNetwork2023,HirschNeuralEmpiricalInterpolation2024}. In this study, we exploit the GPR, detailed further in \cite{GuoReducedOrderModeling2018,OrtaliGaussianProcessRegression2022}.


==> sections/problem.tex <==
%!TEX ROOT=../main.tex
\section{Problem formulation}%
\label{sec:problem_formulation}
The transport-diffusion equation is a linear partial differential equation, which takes the form:
\begin{equation}
\label{eq-transport}
\frac{\partial c}{\partial t} - \nu \Delta c +  \nabla\cdot( \mathbf{u} c )=f;
\end{equation}
where  $c(\mathbf{x}, t):\Omega  \times[0,T) \subset \mathbb{R}^{n} \times \mathbb{R}^{+} \rightarrow
\mathbb{R}$ (with n=2,3) is the unknown function, which can be thought of as the concentration of a pollutant such as NOx. Specifically, the quantity
$c(\mathbf{x}, t) d V$ represents the mass present at time $t$ in an
infinitesimal neighborhood of the point $\boldsymbol{x}$. Consistently, the mass
of pollutant present in volume $V$ at time $t$ is given by :
\begin{equation}
\int_{V} c(\boldsymbol{x}, t) d V.
\end{equation}

Equation \eqref{eq-transport} is known as the convection-diffusion equation because of the physical interpretation of the various terms in it. The diffusive term  "$- \nu \Delta c$"  represents the rate of
change in concentration due to the difference between the average value of $c$
in a neighborhood of $\boldsymbol{x}$  and the value at $\boldsymbol{x}$
itself. In particular, the diffusive flux is given by \textit{Fick's law}:
\begin{equation}
    \mathbf{q} = - \nu \nabla c.
\end{equation}
The minus sign is because the pollutant travels from high-concentration areas to low-concentration ones. The diffusivity constant $\nu > 0$  is dependent on the particular pollutant under consideration and is
assumed to be constant throughout the domain.

The term "$\nabla\cdot( \mathbf{u} c )$", on the other hand, models the convective transport effect, that is, the transport of the pollutant due to the motion of
the fluid in which it is immersed. In particular, the velocity field
$\mathbf{u}$ is given by the resolution of the Navier-Stokes system, which will be presented in the next section.


\subsection{The Navier-Stokes equations}%
\label{sub:the_navier_stokes_equations}
Let $\Omega \subset \mathbb{R}^{n},(n=2,3)$ be a bounded domain and consider the following system of equations, known as the incompressible Navier-Stokes system:
%
\begin{equation}
\label{NavierStokes}
\begin{cases}
\mathbf{u_t}+ \mathbf{\nabla} \cdot (\mathbf{u} \otimes \mathbf{u})- \mathbf{\nabla} \cdot 2 \mu \mathbf{\nabla^s} \mathbf{u}=-\mathbf{\nabla}p &\mbox{ in } \Omega \times [0,T] ,\\
\mathbf{\nabla} \cdot \mathbf{u}=\mathbf{0} &\mbox{ in } \Omega \times [0,T] ,
\end{cases}
\end{equation}
%
where $\boldsymbol{\nabla}^{\boldsymbol{s}}
\mathbf{u}=\frac{1}{2}(\boldsymbol{\nabla} \mathbf{u} + \boldsymbol{\nabla}
^{T}\mathbf{u})$, and $\mu$ is the so-called kinematic viscosity. The unknowns
are represented by the state of the fluid $X=(\mathbf{u},p)$, namely its
velocity and pressure normalized over a constant density. In this
particular setting, the latter can be interpreted as a Lagrange multiplier needed
to impose the incompressibility condition. If we introduce a characteristic
velocity $U_{0}$ and a characteristic length $L$ for the problem under
consideration, we define the following adimensional quantity known as
\textbf{Reynolds number}:
%
\begin{equation}
    \label{Reynolds}
    Re=\frac{U_0 L}{\mu}.
\end{equation}
%
This parameter assumes a fundamental role in fluid dynamics since it scales the nonlinear term when dealing
with the non-dimensionalized version of System \eqref{NavierStokes}. In particular, the Reynolds number makes it possible to
identify different regimes of motion for the problem under consideration.
Indeed, above a problem-specific threshold, the viscous forces are not sufficient
to counteract the inertial ones, and this gives rise to a chaotic motion typical
of the turbulent flows.
%
In order to characterize such turbulent motion, in the present work, we
considered the Reynolds Averaged Navier-Stokes (RANS)\nomenclature{RANS}{Reynolds Averaged Navier-Stokes} equations. This model
involves averaging the quantities of interest over a period chosen to be
smaller than the dynamics of the phenomena ($T_{1}$) under consideration and
larger than the turbulence disturbances ($T_2)$. Each characteristic quantity
of the turbulent motion $\phi$ is decomposed into a time-averaged term
$\overline{\phi}$ and a disturbance or fluctuation $\phi^{\prime}$:
%
\begin{equation}
\begin{aligned}
&\phi=\overline{\phi}+\phi^{\prime}\ ; \\
&\overline{\phi}=\frac{1}{\vartheta} \int_{t}^{t+\vartheta} \phi(\boldsymbol{x},s) ds \ ; \quad T_{1} \le \vartheta \le T_{2} \ .
\end{aligned}
\end{equation}
%
Moreover, the following properties for averaged quantities hold:
%
\begin{equation}
\label{rans-properties}
\overline{\phi^{\prime}}=0 \ , \quad \overline{\overline{\phi}+\phi^{\prime}}=\overline{\phi} \ , \quad \overline{\overline{\phi} \phi^{\prime}}=0 \ , \quad \overline{\phi_{\mathrm{i}}^{\prime} \phi_{\mathrm{j}}^{\prime}} \neq 0 \ .
\end{equation}
%
The Reynolds form of the Navier-Stokes system equation is obtained by taking the
time average of system \eqref{NavierStokes} and exploiting Properties
\eqref{rans-properties}. This procedure leads to the following system:
%
\begin{equation}
\label{Rans}
\begin{cases}
\mathbf{\overline{u}}_{t}+ \mathbf{\nabla} \cdot (\mathbf{\overline{u}} \otimes \mathbf{\overline{u}})+ \mathbf{\nabla} \cdot (\overline{ {\mathbf{u}^{\prime}} \otimes \mathbf{u}^{\prime}})- \mathbf{\nabla} \cdot 2 \mu \mathbf{\nabla^s} \mathbf{\overline{u}}=-\mathbf{\nabla}\overline p &\mbox{ in } \Omega \times [0,T] \  ,\\
\mathbf{\nabla} \cdot \mathbf{\overline{u}}=\mathbf{0} &\mbox{ in } \Omega \times [0,T] \ .
\end{cases}
\end{equation}
%
Specifically, in the momentum equation, the first term represents the average
acceleration of the fluid, and the second term is composed of three parts:
average pressure gradient, viscous stresses caused by the average fluid motion
of laminar nature, and apparent stresses caused by
turbulent fluctuations. The viscous stresses caused by the third term are
grouped within a tensor, called the \textit{Reynolds stress tensor}
$\boldsymbol{\tau}$ , having expression:
%
\begin{equation}
    \boldsymbol{\tau}_{ij} = \overline{ u_{i}^{\prime} u_{j}^{\prime}} \ .
\end{equation}
%
Since the Reynolds stress tensor introduction adds six additional unknowns to the problem, the RANS method needs appropriate turbulence models to be solvable. In particular, for the present work, we used the
$k$-${\epsilon}$ \cite{k-epsilon} model, which consists in adding two PDEs
describing the transport of turbulent kinetic energy ($k$) and turbulent kinetic
energy dissipation rate ($\epsilon$).
For many practical applications, knowledge of the averaged quantities alone may
be sufficient for solving the problem. This approach allows a considerable
computational time reduction since the mean motion scales are much larger than those of turbulent fluctuations.



==> sections/related.tex <==
\section{Related Works}
\label{sec:related}

Reduced order modeling (ROM) techniques have been pivotal in scientific computing for their efficiency in reducing the computational costs associated with solving complex problems modeled by partial differential equations (PDEs). Among various approaches, optimal transport (OT) theory has emerged as a powerful framework due to its capability to preserve the geometric structure of data distributions, making it particularly suited for ROM applications in high-dimensional and nonlinear systems.

Optimal transport, focusing on the geometry of data distributions, provides a
novel perspective in ROM through the use of the Wasserstein distance to quantify
dissimilarities between high-dimensional data sets. This approach has gained
traction within the machine learning community for its ability to effectively
capture the underlying geometry of data spaces. The Sinkhorn algorithm,
introduced by Cuturi \cite{cuturi13}, offers an efficient means to compute the
regularized Wasserstein distance, facilitating its application across various
domains, including generative adversarial networks where the Wasserstein
distance measures discrepancies between true and generated data distributions
\cite{wasserstein-gan}.

In the realm of parametrized PDEs, OT theory's utility is evident in the work by
Mula et al. \cite{mula2020}, which explores ROM using a nonlinear approximation
within the $L^2$-Wasserstein space. This approach is particularly advantageous
for one-dimensional conservative PDEs, demonstrating theoretical and numerical
superiority over traditional linear methods. The extension of this framework to
non-conservative problems \cite{mula2022} and further advancements in employing
Wasserstein barycenters for sparse approximation and structured prediction
\cite{mula2023}, highlight OT's potential in overcoming the limitations of classical ROM techniques, especially for hyperbolic conservation laws.

Additionally, OT has facilitated the development of novel interpolation
techniques for parametric advection-dominated problems. Taddei et
al. \cite{taddei2022} introduced an interpolation method that utilizes OT maps
between Gaussian distributions to identify and track coherent structures via a
maximum likelihood estimator. This approach underscores the adaptability and
effectiveness of OT in handling complex dynamical systems. Furthermore, Blickhan
\cite{blickhan2023registration} proposed a data-driven registration method that employs OT mappings to align solution features, thereby enhancing the approximation capabilities of classical reduced basis methods. This method exemplifies the innovative integration of OT into ROM, opening avenues for methodological developments and applications across various scientific fields.

The integration of optimal transport theory into reduced order modeling presents a promising frontier for efficiently handling parametric PDEs and complex physical systems. By leveraging the geometric fidelity offered by OT, this line of research holds potential for significant methodological advancements and broad applicability in scientific computing and beyond.





==> sections/rom_model.tex <==
\section{A Reduced-Order Modeling Framework for Time-Dependent Problems}
\label{sec:rom-model}

Let us start by considering an abstract PDE problem defined over the domain $\Omega \subset \mathbb{R}^n$ and over time interval of interest $\mathcal{I} = [0, t_f] \subset \mathbb{R}$:
\begin{equation}
\label{eq:abs}
\mathcal{L}(u(t)) = 0, \quad t \in \mathcal{I},
\end{equation}
where $u(t) \in \mathcal{V}$ represents the unknown function within an appropriate function space. The operator $\mathcal{L}$ encompasses the differential operators, boundary conditions, and forcing terms that govern the physical behavior of $u(t)$.
For the numerical solution of \eqref{eq:abs}, classical methods are finite difference, finite element, or finite volume methods.
Once discretized in space, the solution at a specific time instant is denoted by the vector $\boldsymbol{u}_h(t) \in \mathbb{R}^{N_h}$, where $N_h$ represents the number of degrees of freedom.

Let $\mathcal{S} = \left\{\boldsymbol{u}_h(t) \mid t \in \mathcal{I} \right\}$ represent the continuous evolution of $\boldsymbol{u}_h$ as time varies. Let us consider a uniform temporal discretization with $N_T$ time steps. We define the time step size as $\Delta t = \frac{t_f}{N_T}$ and the discrete time points as $t_k = k\Delta t$ for $0 \leq k \leq N_T - 1$. With the introduction of time discretization, we obtain a discretized trajectory set as $
    \mathcal{S}_{h} = \{\boldsymbol{u}_{h}^{k}=\boldsymbol{u}_{h}(t_{k})\}_{k=0}^{N_{T}-1} \subset \mathbb{R}^{N_{h}}$.
Our aim is to study $\mathcal{S}_{h}$ to obtain the best possible approximation of $\mathcal{S}$. Note that we can represent $\mathcal{S}_{h}$ in the form of a \textit{snapshot matrix}:
\begin{equation}\label{eq:snapshots_matrix}
\mathbf{S}=\left[\boldsymbol{u}_{h}^{0}\mid\boldsymbol{u}_{h}^{1}\mid\ldots\mid\boldsymbol{u}_{h}^{N_{T}-1}\right] \in \mathbb{R}^{N_{h} \times N_{T}}.
\end{equation}

To reduce the computational cost associated with fine time discretizations, particularly in applications requiring high-frequency monitoring, we are interested in the development of ROMs that leverage regression and interpolation approaches to approximate the solution \textit{continuously} even when using a large time step $\Delta t$.
We begin by recalling the Proper Orthogonal Decomposition, a linear ROM strategy widely used in ROMs. This approach will be exploited both as a metric to compute performance and, together with a regression strategy, to learn residuals.

\input{sections/pod}


==> sections/temp.tex <==
In our checkpoint selection process, we vary the number of checkpoints $N_c$ while maintaining a constant total number of synthetic snapshots $N_{\text{tot}} = 1021$. For each $N_c$, we adapt $N_{\text{synth}}^i$ according to:

\begin{equation}
N_{\text{synth}}^i = \left\lfloor\frac{N_{\text{tot}} - N_c}{N_c - 1} \right\rfloor .
\end{equation}

Figure \ref{fig:synthetic-evolution} illustrates the evolution of synthetic solutions as $N_c$ varies for $\Delta t_{\text{train}} = 0.1$ s. With increasing $N_c$, the interpolated trajectory becomes more physically meaningful.

\begin{figure}[ht]
	\centering
    %\includegraphics[width=\textwidth]{barycentric_field_evolution.png}
	\caption{Evolution of synthetic solutions for the rising thermal bubble as the number of checkpoints ($N_c$) varies.}
	\label{fig:synthetic-evolution}
\end{figure}

To assess computational efficiency, we introduce a speed-up factor, defined as the ratio between the time for executing steps 1-3 of our method and the FOM time for collecting $\mathcal{S}_{\text{test}}$.
Figure \ref{fig:speedup} shows this factor decreasing with increasing $N_c$, but remaining advantageous (>1) for $N_c < 171$.

\begin{figure}[ht]
    \centering
    [Placeholder for speedup factor plot]
    \caption{Speed-up factor $S$ vs. number of checkpoints $N_c$ for the thermal bubble test case.}
    \label{fig:speedup}
\end{figure}

Figure \ref{fig:alpha_global} demonstrates how $\alpha_{\text{global}}(\cdot,\mathcal{M})$ approaches the linear mapping $\mathcal{L}$ as $N_c$ increases, indicating that $\mathcal{M}$ effectively captures the near-linear relationship between physical time and interpolation parameter for sufficiently large $N_c$.

\begin{figure}[ht]
\centering
[Placeholder for $\alpha_{\text{global}}$ vs. time plot]
\caption{Global interpolation parameter $\alpha_{\text{global}}$ vs. time for different mapping strategies and numbers of checkpoints.}
\label{fig:alpha_global}
\end{figure}

Finally, Figure \ref{fig:reconstruction_error} shows the mean reconstruction error $\overline{E}_{\mathcal{M}}$ as a function of $N_c$ for different $\Delta t_{\text{train}}$. The error decreases with increasing $N_c$, eventually plateauing at the discretization error $E_{\text{disc}}$, highlighting the inherent limitation imposed by the temporal discretization of the training data.

\begin{figure}[ht]
\centering
[Placeholder for mean reconstruction error plot]
\caption{Mean reconstruction error $\overline{E}_{\mathcal{M}}$ vs. number of checkpoints $N_c$ for different $\Delta t_{\text{train}}$.}
\label{fig:reconstruction_error}
\end{figure}


==> sections/thermal-bubble.tex <==
\subsection{Rising Thermal Bubble}
\label{subsec:thermal-bubble}
\graphicspath{{Images/thermal_bubble/}}

The computational domain for this benchmark is $\Omega = [\SI{0}{\meter}, \SI{5000}{\meter}] \times [\SI{0}{\meter}, \SI{10000}{\meter}]$ in the $xz$-plane. We discretize the domain using a uniform structured mesh with mesh size of $h = \Delta x = \Delta z = \SI{125}{\meter}$, resulting in a $40 \times 80$ grid and $N_h = 3200$.

The initial conditions are defined as follows:
\begin{equation}
\left\{
\begin{aligned}
\theta_s &= \SI{300}{\kelvin}, \\[6pt]
\theta_0 &= \begin{cases}
    \theta_s + 2\left[1 - \frac{r}{r_0}\right] & \text{if } r \leq r_0 = \SI{2000}{\meter} \\
    \theta_s & \text{otherwise}
\end{cases} ,\\[6pt]
\rho_0 &= \frac{p_g}{R\theta_0}\left(\frac{p}{p_g}\right)^{c_v/c_p} \text{ with } p = p_g\left(1 - \frac{gz}{c_p\theta_0}\right)^{c_p/R}, \\[6pt]
\u_0 &= \mathbf{0}, \\[6pt]
\end{aligned}
\right.
\end{equation}
where $r = \sqrt{(x - x_c)^2 + (z - z_c)^2}$ is the distance from the center of the perturbation $(x_c, z_c) = (\SI{0}{\meter}, \SI{2000}{\meter})$. The values of constants $p_g$, $g$, $c_p$, and $R$ are as given in Sec.~\ref{sec:FOM}. This perturbation in the potential temperature field affects the pressure and density fields through the adiabatic balance equation \eqref{eq:potential_temperature} and the equation of state \eqref{eq:state_potential}, respectively.

\begin{figure}[ht]
	\centering
    \includegraphics[width=.8\textwidth]{solution_evolution.pdf}
	\caption{Evolution of the potential temperature perturbation field $\theta'$ for the rising thermal bubble test case.}
	\label{fig:thermal-bubble-evolution}
\end{figure}

We impose impenetrable, free-slip boundary conditions on all domain boundaries. The simulation is run for a total time of $t_f = \SI{1021}{\second}$. During this time interval, the warm bubble rises due to buoyancy forces and evolves into a characteristic mushroom-like shape as a result of shear stresses at its edges. See Figure~\ref{fig:thermal-bubble-evolution}.

For the numerical simulation, we use the artificial viscosity $\mu_a = \SI{15}{\meter\squared\per\second}$ and Prandtl number $\Pr = 1$, as suggested in \cite{Ahmad2006}. These values are chosen ad hoc to stabilize the numerical simulation and ensure the resolution of the main flow features without excessive diffusion.


We generate the reference solution $\theta'_{\text{ref}}(t)$ using $\Delta t_{\text{ref}} = \SI{0.005}{\second}$. For training, we employ coarser time steps $\Delta t_{\text{train}} \in \{\SI{0.01}{\second}, \SI{0.1}{\second}, \SI{1}{\second}\}$. The sets of training and test points are defined as:
\begin{equation*}
\begin{aligned}
    \mathcal{T}_{\text{train}} &= \{t^k_{\text{train}} = k \Delta t_{\text{save}} \mid k = 1, ..., N_T\}, \\
    \mathcal{T}_{\text{test}} &= \{t_{\text{test}}^j = j + (0.05 \pm \Delta t_{\text{test}}) \mid j = 1, ..., N_T\},
\end{aligned}
\end{equation*}
where $\Delta t_{\text{save}} = \SI{1}{\second}$ and $N_T = 1021$.

Table \ref{tab:disc_error} reports
the discretization error $\overline{E}_{\text{disc}}(\Delta t_{\text{train}})$ for each $\Delta t_{\text{train}}$, along with execution times and time ratios relative to the reference case.
The reference case, with $\Delta t = \SI{0.005}{\second}$, has an execution time of \SI{659.76}{\second}. As expected, when going from $\Delta t = \SI{1}{\second}$ to $\Delta t = \SI{0.1}{\second}$, the discretization error decreases. However, the discretization error remains of the same order of magnitude when further reducing the time step to $\Delta t = \SI{0.01}{\second}$, suggesting that the error due to time discretization becomes negligible with respect to the spatial discretization error.
For this reason, we will show only the results for $\Delta t = \SI{0.1}{\second}$ and $\Delta t = \SI{1}{\second}$ in the subsequent analysis.
Table \ref{tab:disc_error} also highlights the computational efficiency gained by using larger time steps. For instance, the simulation with $\Delta t = \SI{1}{\second}$ runs approximately 46 times faster than the reference case, while still maintaining a reasonable level of accuracy.


\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        $\Delta t_{\text{train}}$ & $\overline{E}_{\text{disc}}(\Delta t_{\text{train}})$ & Execution Time & Time Ratio \\
        \hline
        \SI{1}{\second}  & 3.88e-02 & \SI{14.18}{\second} & 46.53 \\
        \SI{0.1}{\second}  & 8.53e-03 & \SI{45.54}{\second} & 14.81 \\
        \SI{0.01}{\second} & 9.63e-03 & \SI{332.19}{\second} & 1.99 \\
        \hline
    \end{tabular}
    \caption{Discretization error $\overline{E}_{\text{disc}}(\Delta t_{\text{train}})$, execution time, and time ratio relative to the reference case (with $\Delta t = \SI{0.005}{\second}$) for different training time steps.}
    \label{tab:disc_error}
\end{table}


In the checkpoint selection process, we vary the number of checkpoints $N_c$ while maintaining a constant total number of synthetic snapshots $N_{\text{tot}} = 1021$. For each $N_c$, we adapt $N_{\text{synth}}$ according to:
\begin{equation*}
N_{\text{synth}} = \left\lfloor\frac{N_{\text{tot}} - N_c}{N_c - 1} \right\rfloor.
\end{equation*}
Figure \ref{fig:synthetic-evolution} illustrates the evolution of synthetic solutions as the number of checkpoints varies for $\Delta t _{\text{train}}= \SI{1}{\second}$. Note that checkpoints act as forced passage points for the interpolated field. For instance, when $N_c = 2$, the interpolant follows a path that causes the supports to move along the diagonal connecting the initial condition to the final solution, resulting in a trajectory
of limited physical relevance. However, as we increase the number of checkpoints, we constrain the solution to follow a progressively more physically meaningful trajectory.
\begin{figure}[ht]
    \centering
    \includegraphics[width=.85\textwidth]{barycentric_field_evolution.pdf}
    \caption{Evolution of synthetic solutions for the rising thermal bubble as the number of checkpoints $N_c$ varies. The images demonstrate how increasing $N_c$ leads to more physically relevant interpolated trajectories.}
    \label{fig:synthetic-evolution}
\end{figure}

Table \ref{tab:computation_time} shows the percentage breakdown of computation time for different steps of our method, as well as the total computation time, for different numbers of checkpoints.
We see that Steps 2-3, which involves solving the OT problems in \eqref{eq:step2}, carry the majority of the computational cost, especially as the number of checkpoints increases. However, these problems are entirely independent of each other, and thus amenable to complete parallelization\footnote{In our current implementation, we have not fully leveraged this parallelization potential, as the computations were not performed on a distributed cluster.}.

\begin{table}[htbp]
\centering
\begin{tabular}{|l|cccccc|}
\hline
 & \multicolumn{6}{c|}{Number of Checkpoints ($N_c$)} \\
 & 2 & 11 & 31 & 61 & 103 & 171 \\
\hline
Step 2-3 (\%) & 81.74 & 90.79 & 96.80 & 98.28 & 99.09 & 99.44 \\
Step 5 (\%)   & 18.25 & 9.20  & 3.20  & 1.72  & 0.91  & 0.56 \\
Total Time (s) & 10.44 & 30.54 & 91.78 & 178.26 & 309.99 & 505.17 \\
\hline
\end{tabular}
\caption{Computation time breakdown for different numbers of checkpoints ($N_c$) with time step $\Delta t = \SI{1.0}{\second}$.}
\label{tab:computation_time}
\end{table}

To assess the computational efficiency of our approach for the \textit{online phase}, we introduce the concept of \textit{speed-up}. This metric is defined as the ratio between the reference FOM time (for $\Delta t_{\text{test}} = \SI{0.005}{\second}$) and the time required for Step 5, which represents the online inference phase of our method. It is important to note that we are primarily comparing the online inference times, as this phase utilizes precomputed OT plans, resulting in a simple matrix-vector multiplication with relatively low computational cost. Figure \ref{fig:speed_up} illustrates how the speed-up varies with the number of checkpoints $N_c$ for different time steps $\Delta t$. The speed-up decreases with increasing $N_c$, but remains advantageous \((\mathcal{O}(10^2))\) for all considered \(N_c\) values.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\textwidth]{speed_up_plot.pdf}
    \caption{Speed-up  factor as a function of the number of checkpoints $N_c$ for the rising thermal bubble test case.}
    \label{fig:speed_up}
\end{figure}

To better understand the relationship between physical time and the interpolation parameter, in Figure \ref{fig:alpha_global} we examine the behavior of the global interpolation parameter $\alpha_{\text{global}}(\cdot,\mathcal{M})$ as a function of time for different numbers of checkpoints.
We observe that increasing the number of checkpoints causes the $\mathcal{M}$ mapping to progressively approach the linear mapping $\mathcal{L}$, as explained in Remark \ref{remark1}.

\begin{figure}[ht]
\centering
\includegraphics[width=1\textwidth]{alpha_global_plot.pdf}
\caption{Global interpolation parameter $\alpha_{\text{global}}(\mathcal{M})$ in red and its deviation in blue over time for $N_c = 2$ (left), $N_c = 11$ (center), $N_c = 171$ (right).}
\label{fig:alpha_global}
\end{figure}

Figure \ref{fig:reconstruction_error} shows the generalization errors for both mappings $\mathcal{M}$ and
$\mathcal{L}$ and selected numbers of checkpoints and time step sizes. $E_{\text{gen}}$ is made up of two components: one from displacement interpolation and the other
from temporal discretization. The interpolation error decreases with increasing $N_c$, showing oscillatory behavior between checkpoints. Local minima occur near checkpoints, reflecting reduced error at known data points. As $N_c$ increases, this error decreases,
lowering the overall $E_{\text{gen}}$ until the
time discretization error dominates.

Figure \ref{fig:mean_error} provides a comprehensive view of the mean interpolation and generalization errors as functions of $N_c$ for both mappings $\mathcal{M}$ and $\mathcal{L}$ and different $\Delta t$ values.
Only $E_{\text{interp}}$ for $\Delta t = \SI{1}{\second}$
is presented as it remains consistent across $\Delta t$, indicating robustness to temporal discretization.
This can be attributed to the underlying displacement interpolation capability: since the checkpoints are similar for different $\Delta t$, the interpolant behavior within each interval remains comparable.

Let us summarize the results shown so far.
The mean interpolation error $\overline{E}_{\text{interp}}$ decreases monotonically with increasing $N_c$ for both mappings, with $\mathcal{M}$ consistently outperforming $\mathcal{L}$, especially for lower values of $N_c$, when the deviation from linearity is significant, as shown in Figure \ref{fig:alpha_global}. The mean generalization error $\overline{E}_{\text{gen}}$ exhibits a similar trend, but saturates at the underlying time discretization error $\overline{E}_{\text{disc}}$ for each $\Delta t$.  This saturation highlights an important characteristic of our method: by increasing $N_c$, we can effectively reduce the error associated with the displacement interpolation representation, but we are ultimately bounded by the inherent temporal discretization error of the training data.
Thus, our method is able to achieve optimal accuracy within the constraints of the temporal resolution
of the training data.


\begin{figure}[ht]
\centering
\includegraphics[width=1\textwidth]{generalization_error_plot.pdf}
\caption{Generalization error $E_{\text{gen}}$ over time $t$ for both mappings $\mathcal{M}$ and $\mathcal{L}$ and different values of $N_c$ and $\Delta t$. Note that the scale of the vertical axis varies in each subplot.}
\label{fig:reconstruction_error}
\end{figure}

%\begin{figure}[ht]
%\centering
%\includegraphics[width=1\textwidth]{interpolation_error_plot.pdf}
%\caption{Interpolation error $E_{\text{interp}}$ vs. time $t$ for different $N_c$ and $\Delta t$.}
%\label{fig:interpolation_error}
%\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=1\textwidth]{error_plots_mean.pdf}
\caption{Mean interpolation error $\overline{E}_{\text{interp}}$ (left) and mean generalization error $\overline{E}_{\text{gen}}$ (right)
for both mappings $\mathcal{M}$ and $\mathcal{L}$
vs. the number of checkpoints $N_c$ for different time step sizes $\Delta t$.}
\label{fig:mean_error}
\end{figure}

\subsubsection*{POD Analysis of Synthetic Datasets}

To further evaluate the effectiveness of our data augmentation strategy, we performed POD on two datasets. The first is the synthetic snapshot matrix $\mathbf{S}_{\text{synth}} \in \mathbb{R}^{N_h \times N_\text{tot}}$, as defined in Sec.~\ref{sec:ot_rom_framework}, which includes both the original checkpoints and the interpolated states. The second is the checkpoint snapshot matrix $\mathbf{S}_{\text{check}} \in \mathbb{R}^{N_h \times N_c}$, containing only the $N_c$ checkpoints selected from the FOM trajectory $\mathcal{S}_h$.
For both cases, we set an energy threshold of 99.99\% to determine the number of POD modes to retain. This high threshold ensures that we capture almost all of the system's energy in our reduced basis.
Let $\mathbf{U}_{\text{synth}}$ and $\mathbf{U}_{\text{check}}$ denote the POD bases obtained from $\mathbf{S}_{\text{synth}}$ and $\mathbf{S}_{\text{check}}$, respectively. We compute
the projection errors for both the training and test datasets onto these bases, which for a given snapshot $\boldsymbol{u}_h(t)$ onto a basis $\mathbf{U}$ is given as\footnote{Here, $\boldsymbol{u}_h(t)$ denotes the vector of degrees of freedom associated with the discretized solution at time $t$.}:
\begin{equation}\label{eq:errproj}
E_{\text{proj}}(\boldsymbol{u}_h(t), \mathbf{U}) = \frac{\|\boldsymbol{u}_h(t) - \mathbf{U}\mathbf{U}^T\boldsymbol{u}_h(t)\|_2}{\|\boldsymbol{u}_h(t)\|_2}.
\end{equation}
We compute $E_{\text{proj}}$ in \eqref{eq:errproj} for both $\mathcal{S}_{\text{train}}$ and $\mathcal{S}_{\text{test}}$, using $\mathbf{U}_{\text{synth}}$ and $\mathbf{U}_{\text{check}}$.

Figure \ref{fig:pod_projection_errors} presents the projection errors for both $\mathbf{U}_{\text{synth}}$ and $\mathbf{U}_{\text{check}}$ across different values of $N_c$ and $\Delta t$. For $\Delta t = \SI{1}{\second}$, the projection error for $\mathbf{U}_{\text{synth}}$ becomes comparable to $\overline{E}_{\text{disc}}$ with as few as 3 checkpoints, while for $\Delta t = \SI{0.1}{\second}$ it takes 11 checkpoints.
This difference can be attributed to the finer temporal resolution capturing more detailed dynamics
and hence necessitating a larger number of checkpoints to adequately represent the solution manifold,
and the lower $\overline{E}_{\text{disc}}$ threshold for $\Delta t = \SI{0.1}{\second}$ . We see that
$\mathbf{U}_{\text{synth}}$ consistently outperforms $\mathbf{U}_{\text{check}}$, especially for lower $N_c$
values, with this superiority more pronounced for $\Delta t = \SI{1}{\second}$. As $N_c$ increases, errors for both bases converge to similar values.
This happens earlier for $\Delta t = \SI{0.1}{\second}$, suggesting that, for sufficiently high $N_c$, the additional information from synthetic snapshots becomes less critical.

\begin{figure}[htpb]
\centering
\includegraphics[width=1\textwidth]{pod_projection_errors.pdf}
\caption{Projection errors for POD bases derived from synthetic and checkpoint datasets for $\Delta t = 1$ (left) and $\Delta t = 0.1$ (right).}
\label{fig:pod_projection_errors}
\end{figure}

